Navigating AI Fallibility: Examining People's Reactions and Perceptions of AI after Encountering Personality Misrepresentations

Many hyper-personalized AI systems profile people's characteristics (e.g., personality traits) to provide personalized recommendations. These systems are increasingly used to facilitate interactions among people, such as providing teammate recommendations. Despite improved accuracy, such systems are not immune to errors when making inferences about people's most personal traits. These errors manifested as AI misrepresentations. However, the repercussions of such AI misrepresentations are unclear, especially on people's reactions and perceptions of the AI. We present two studies to examine how people react and perceive the AI after encountering personality misrepresentations in AI-facilitated team matching in a higher education context. Through semi-structured interviews (n=20) and a survey experiment (n=198), we pinpoint how people's existing and newly acquired AI knowledge could shape their perceptions and reactions of the AI after encountering AI misrepresentations. Specifically, we identified three rationales that people adopted through knowledge acquired from AI (mis)representations: AI works like a machine, human, and/or magic. These rationales are highly connected to people's reactions of over-trusting, rationalizing, and forgiving of AI misrepresentations. Finally, we found that people's existing AI knowledge, i.e., AI literacy, could moderate people's changes in their trust in AI after encountering AI misrepresentations, but not changes in people's social perceptions of AI. We discuss the role of people's AI knowledge when facing AI fallibility and implications for designing responsible mitigation and repair strategies.

==> deleted.tex <==


% \subsection{People's Reactions and Perceptions of Faulty AI} 
% % Much research has been conducted to understand how people perceive AI agents differently after encountering AI failures, most of which had been done in the area of human-robot interaction. Prior work established that encountering robot failures would significantly lower people's perceptions of the robot~\cite{honig2018understanding} in terms of robots' trustworthiness~\cite{salem2015would,law2017wizard,roesler2020effect}, perceived intelligence~\cite{takayama2011expressing}, perceived likeability~\cite{mirnig2017err}, anthropomorphism~\cite{salem2015would}, reliability~\cite{salem2015would}, and ease of use~\cite{de2023we}. However, some of these results were inconclusive given that other research has suggested that AI mistakes could be considered as a human-like characteristics, and therefore could make the interactions more engaging and natural, mitigating the potential negative effect AI mistakes might have on users' perceptions of the AI~\cite{honig2018understanding,buhrke2021making,mirnig2017err}. For instance,~\citeauthor{mirnig2017err} [2017] did not find a significant difference in perceived intelligence and anthropomorphism between participants who interacted with faulty robots vs. flawless robots~\cite{mirnig2017err}; studies also suggested that robot failures might make users' interaction experience more pleasurable~\cite{mirnig2017err,honig2018understanding,gompei2015robot} and more engaged~\cite{honig2018understanding,law2017wizard}. Some prior work has offered explanations that people's perception after encountering robot failures might be attributed to a number of factors such as types of failures, failure severity, or the nature of the task (e.g., formal workplace or social and personal)~\cite{sarkar2017effects,honig2018understanding,rossi2017timing}. Therefore, it is important to examine how people's perceptions changed after encountering AI mistakes in different context to better inform the human-centered design of AI's repair and recovery strategies. 

% % There is also a growing body of research in HCI focused on studying people's reactions and attitudes of towards AI algorithms such as recommendation algorithms, with ``trust'' as the core concept of interest. Much research in this area suggested that people had a tendency to overtrust AI~\cite{oh2022you,banas2022machine,kapania2022because} and to attribute more credibility to AI~\cite{kapania2022because,edwards2016robots} comparing to human agents--- some even pointed out that AI was considered as an authority figure that could influence people's behaviors without needing to provide adequate evidence~\cite{kapania2022because}. In their interview study on people's perceptions and attitudes of AI in India,~\citeauthor{kapania2022because} [2022] found that people seemed to have a high tolerence of AI failures, with some displaying tendencies of forgiving and justifying AI misfires, or even blame themselves or others for AI's mishaps~\cite{kapania2022because}. Many researchers attributed this tendency to overtrust AI to people's machine heuristics~\cite{sundar2020rise}: the belief that machines are objective, emotionless, and logical entities without feelings, therefore more trustworthy comparing to humans~\cite{sundar2020rise}. 

% % However, only a few work has empirically studied people's reactions and attitudes towards AI mistakes, and suggested additional, sometimes contradictory findings. For example, instead of overtly positive view and reliance on AI,~\citeauthor{hsu2021attitudes} [2021] found that students perceived AI autograders as unfair and harmful due to their over-estimation of the AI's error rate~\cite{hsu2021attitudes}. While~\citeauthor{oh2022you} [2022] corroborated with findings from prior literature that people tended to have greater trust and more positive attitudes towards machine-generated recommendations comparing to human-generated recommendations, they also found that people's trust and general attitudes declined quickly after users saw machines made mistakes (also known as the phenomenon of algorithm aversion~\cite{dietvorst2015algorithm}). This suggested that multiple heuristics could exist and interact together to shape people's perceptions and attitudes towards AI after encountering AI mistakes. 


% % \cite{hsu2021attitudes}: understanding students' attitudes, knowledge, and perception. Misalignments between students' folk theories about the autograder and how it actually worked. Perceived the autograder as unfair and harmful due to incorrect estimation.

% % \cite{oh2022you}: people showed more positive attitude toward a machine recommender than a human recommender. Machine heuristic: the higher the users perceive the rec as machine, the more positive attitudes. Automation bias induces people to adhere to automated decision authorities. Over-credence on recommendation algorithm. 

% % \cite{dietvorst2015algorithm}: algorithm aversion: people quickly lose confidence in algorithm than human forecasters after seeing them make the same mistake. 

% % \cite{banas2022machine}: Second, heuristic preference in machines and crowds matters more when the corresponding fact-checking agent labels a claim as true rather than false; this result is consistent with the idea that people are more tolerant of agents incorrectly fact-checking a story as true (false positives) than they are for the reverse when a story is incorrectly marked as false (false negatives). Third, system transparency explanations do not appear to interact with heuristics and agents’ assessments to affect veracity judgments. Overall, these results provide a nuanced understanding of how people rely on AI and human agents’ judgments and their own heuristic biases to make decisions about the veracity of truth-ambiguous information.

% % \cite{milani2023navigates}: assessments of human likeness are influenced by stereotyped beliefs about AI capabilities. Different people have different interpretations of what is human-like behavior. 

% % \cite{kapania2022because}: case of AI authority: forgiveness, self-blame. High tolerence for system misfires. Inclination to forgive or justify wrong decisions or incorrect recommendations. Blamed themselves for receiving an adverse outcome. View AI as machines, emotionless, logical entities. 

% % \cite{edwards2016robots}: teacher as robot was perceived as most credible. Machines are perceived as more objective, less capable of feeling and relating. 

% % \cite{wenzel2023can}: failed automatic speech recognition could lead to higher self-consciousness, lower marginalized groups' self-esteem and positive affect, less favorable ratings of the technology. 


% % - Trust and Machine Heuristic, view AI as an authority. Algorithm aversion -> transparency and XAI


% \subsection{Interacting with Hyper-Personalized AI Systems}
% % With the advancement of algorithms to detect and profile people's personal traits such as their emotions~\cite{wang2020sensing,disalvo2022reading,hollis2018being} and personality characteristics~\cite{gou2014knowme,warshaw2015can,liao2021crystal}, there has been some work conducted in HCI to understand people's reactions and concerns about this type of hyper-personalized AI systems. Prior work found that most users found their AI-generated personality profiles to be ``creepily accurate''~\cite{gou2014knowme,warshaw2015can,liao2021crystal,kim2020understanding}, which was cited as evidence in early studies as proof for feasibility and accuracy of personality recognition algorithms~\cite{gou2014knowme}. However, later qualitative research showed that, even though AI-generated personality profiles are about the users themselves, many users considered AI as an ``expert'' and better than them at recognizing their personalities and/or emotions~\cite{warshaw2015can,hollis2018being}:~\citeauthor{warshaw2015can} found that people felt unqualified to modify their personality profile generated by automated personality recognition algorithm due to their over-trust in the ``expert'' algorithm;~\citeauthor{hollis2018being} echoed this finding and added further that some users even overrode their personal judgements about their emotions, and believed that the AI algorithm was capable of identifying their ``hidden self'' and had privileged information about their emotions. 

% % Despite people's trust in AI-generated profiles about them, when it comes to sharing these AI-generated emotion or personality profiles about them, prior research identified a somewhat contradictory attitudes and opinions. Some suggested that users still wanted control over modifying their profile and traits before sharing due to concerns over others' misinterpretations of AI-inferred traits about them~\cite{gou2014knowme}; however, others have found that users felt compelled to share despite their reservations about sharing given that they wouldn't want others to think they had something to hide~\cite{warshaw2015can}.

% % To understand people's reasoning behind this myriad of attitudes and reactions,~\citeauthor{liao2021crystal} [2021] conducted qualitative interviews to pinpoint people's folk theories about automated personality recognition systems. Consistent with prior work on people's folk theories and beliefs about AI algorithms~\cite{eslami2015always,eslami2016first,devito2018people}, they found that people's reactions and attitudes were largely based on people's folk theories; for example, people with limited folk theories about the data source, data scope, and personalization of output about the AI algorithm allowed them to dismiss AI's personality inferences as less threatening~\cite{liao2021crystal}.~\citeauthor{kim2020understanding}[2020] further added that factors such as the data driven aspect of the system, users' self-perception of their own personality, and the ambiguity around how the system works could all influence people's trust in the result of AI-generated personality inferences. 


% % \cite{gou2014knowme}: two-part study with 256 participants. Showed there is a feasibility of deriving personality traits from social media. Over 61.5\% users are wiling to share their derived traits in the workplace and various factors (what to share, whom to share, and when to share) could influence their sharing preferences. Participants consider it as very personal information. Desire of system transparency on system usage and function. Highlighted two user concerns: others' misinterpretation of the user's inferred personal triats, and users wanting control to modify their profile and traits. 

% % \cite{warshaw2015can}: Qualitative study of people's reactions to a working hyper-personal analytics system. Our results reveal a paradox. Participants found their personal traits profiles creepily accurate and did not like sharing them in many situations. However, they felt pressured by the social risks of not sharing and showed signs of learned helplessness, leading them to share despite their misgivings. Further they felt unqualified to significantly moify their profile contents due to a surprising trust in the expert algorithm. 

% % \cite{hollis2018being}: we explore how people construe algorithmic interpretations of emotional data in personal informatics systems. Users still deferred to feedback and their perceived emotions were significantly influenced by feedback frames. Some users overrode personal judgments, believing the system had access to privileged info about their emotions. Risks of users trusting systems that seemingly unlock hidden aspects of the self.  

% % \cite{kim2020understanding}: participants' trust in results was affected by the following factors: (1) data driven aspect of the system, (2) self-perception of their own personality, and (3) ambiguity around how the system works. 

% % \cite{liao2021crystal}: this study examines how people construct ``snap'' folk theories about the ways personality algorithms operate as well as how they react when shown their outputs. Through qualitative interviews (n = 37) with people after being presented with their own profile, this study identifies a series of folk theories that people came up with to explain the personality algorithm across four dimensions (data source, scope, collection process, and outputs). In addition, this study examined how those folk theories contributed to certain reactions, fears, and justifications people had about the algorithm. Personalization of output: astrology to omniscience. The limited folk theories about... alowed people to dismiss it as less threatening. People's reactions depends on the kind of folk theories they formed (limited to advanced). Worried issues arising from inaccuracy. People blame themselves about data source

% % \cite{devito2018people}: form folk theory based on endogenous info (originates with the platform itself) and exogenous info: originate outside the platform. Folk theories are malleable. Show that the relationship between audience and self is no longer direct, as self-presentation used to be like described by Goffman. Web skills are related to people's folk theories and information source that they seek (high web skill tend to seek endogenous info)



% \subsection{AI-Facilitated Impressions in Human Community}
% % - People's relationships and perceptions of each other can now be mediated through AI algorithms.Folk theories and self-presentations. ~\cite{eslami2015always,eslami2016first}
% % AI-mediated social interactions such as online dating algorithms. 

% % - AI-mediated communication.

% % - But none of these examined AI-mediated impressions in the context of team-matching. This is a formal and relatively professional context and setting, yet based on people's most personal traits and characteristics. 

% % People's self-perceptions and relationships with others can be influenced and mediated by AI algorithms. 

% Our daily interactions and communications are heavily mediated through AI algorithms nowadays. As~\citeauthor{devito2018people} has pointed out in managing AI-mediated impressions in human communities, the relationship between ourselves and the audience are no longer as direct as~\citeauthor{goffman2016presentation} described. Much research has been done to understand and explore people's practices of managing their impressions through social media platforms that are powered by AI algorithms~\cite{karizat2021algorithmic,devito2017platforms,eslami2015always,eslami2016first}. This body of literature has suggested that people not only leverage platform affordances and their folk theories of the platform algorithms to build their self-presentations on the platforms~\cite{devito2017platforms,karizat2021algorithmic}, but also perceive of others and their relationships to others based on algorithm behaviors~\cite{eslami2015always,eslami2016first}. For instance, in their investigation of people's understanding of Facebook recommendation algorithms,~\citeauthor{eslami2015always} found that people formed misperceptions about their friends whose posts never showed up in their feed due to lack of understanding of the recommendation algorithm, which led them to make inferences about their relationships with that person. In the age of AI-mediated interactions, we have begun to see ourselves and others through the filtered lens of algorithms, which unfortunately often presented as a black box to people.

% The burgeoning area of AI-Mediated Communication (AI-MC)~\cite{hancock2020ai}, which referred to communications that are augmented, optimized, or generated by AI, has also offered implications of how AI-facilitated impressions could influence people's interpersonal communications and dynamics. Prior work has suggested that self-presentations or impressions, when knowingly augmented by AI, can decrease its perceived trustworthiness~\cite{jakesch2019ai} and undermine social attractions between people~\cite{mieczkowski2021ai}. However, some work also pointed out that AI could be perceived as having agency when facilitating human-human communications, leading people to transfer their impression of the AI to human~\cite{li2023impression} or having the AI acted as a moral crumble zone for humans to blame for communication breakdowns~\cite{hohenstein2020ai}.


% % \cite{karizat2021algorithmic}: participants changed their behaviors to shape their algorithmic identities to align with how they understood themselves. We argue the relationship between users' algorithmic folk theories and identity are consequential for social media platforms, as it impacts users' experiences, behaviors, sense of belonging, and perceived ability to be seen, heard, and feel valued by others as mediated through algorithmic systems. 

% % \cite{devito2018people}: form folk theory based on endogenous info (originates with the platform itself) and exogenous info: originate outside the platform. Folk theories are malleable. Show that the relationship between audience and self is no longer direct, as self-presentation used to be like described by Goffman. Web skills are related to people's folk theories and information source that they seek (high web skill tend to seek endogenous info)

% % \cite{devito2017platforms}: affordances of social media platforms that affect how people build their self-presentations. 

% % \cite{eslami2015always}: observing the output surprised some unaware participants by revealing misperceptions about their friends whose stories were not shown in the news feed at all. Use it to make inferences about their relationships. 

% % \cite{eslami2016first}: interviews revealed 10 folk theories of automated curation. 






% \section{Study 2: Examining the Impact of AI Misrepresentation on Students' Perception of AI}
% To examine the impact of AI misrepresentation on students' perception of AI (RQ3), we conducted a two-part longitudinal survey study on the Prolific crowdsourcing platform to solicit a larger and more diverse sample. We deployed study 2 by following a similar procedure as study 1 by first deploying a preliminary survey, then after a week, followed by a experiment survey to show participants SAMI's inferences and measured their perception changes of SAMI. We also made some minor revisions to the measurements based on our findings and observations from study 1. In study 2, we also further examined AI literacy as a possible moderating factor on students' changes in perceptions of AI after encountering AI misrepresentation. Specifically, study 2 aimed at answering two research questions to examine the impact of AI misrepresentation on students' perception of AI:

% \begin{table}[h]
% % \sffamily
% \centering
% % \footnotesize
% \vspace{-0.5em}
% \begin{tabular}{@{}l@{}p{0.92\columnwidth}@{}}
%     \textbf{RQ 3.1: } & What is the effect of AI misrepresentation on students' trust and social perceptions of the AI?  \\
%     \textbf{RQ 3.2: } & How does students' level of AI literacy moderate the effect of changes in students' perception of AI after encountering AI misrepresentation? \\
%     % \bottomrule
% \end{tabular}
% \vspace{-0.9em}
% \end{table}


% \subsection{Study 2 Study Design}
% \subsubsection{Study 2 Procedure} 
% Study 2 procedure largely remained the same as the study procedure of study 1, except that the semi-structured interview portion was removed in study 2 given that the aim of study 2 was to collect a large sample to quantitatively examine the impact of AI misrepresentation on students' perception of AI. 

% Similar to study 1, we first deployed a preliminary survey on the Prolific platform. Participants were told that the goal of this longitudinal study was to understand people's perception of a team-matching AI agent. In the preliminary survey, participants were asked to write a paragraph to introduce themselves to SAMI, filled out the 44-item Big Five personality test, a measurement of AI literacy and a measurement of their general attitudes toward AI. Participants then provided their demographic information, their level of study, major or background, as well as the number of team projects they have been involved with and their overall experience with their past team projects at school. All the participants were compensated with \$3 USD for their time after successfully completing the preliminary survey. The median completion time for the preliminary survey is about 11 min. 

% 250 prolific participants filled out our preliminary survey on Qualtrics. After manually checking through their survey responses one by one, we removed seven participants whose self-introduction paragraph were suspected to be generated by ChatGPT. We then wrote a python script to fabricate SAMI's inferences for the 243 remaining participants, following the same inference fabrication procedure and guideline that we described in section~\ref{fabrication}. All the fabricated inferences generated must follow the strict 60\% positive inference and 40\% negative inference ratio, which removed 21 participants in the participant pool given that these 21 participants' fabricated inferences were either too positive or too negative based on how they filled out their personality measurement. This resulted in 222 participants remaining and we invited all 222 participants back to participate in the second survey of study 2, which we refer to as experiment survey. Participants who were invited back to complete the experiment survey was randomly assigned to either the accurate condition or the inaccurate condition. Given our emphasis on AI misrepresentation, we assigned more participants to the ianccurate condition than the accurate condition--- we ended up assigning 157 participants to the inaccurate condition and 65 participants to the accurate condition. 

% The experiment survey, hosted on Qualtrics, was lightly modified based on the survey measurement used at the beginning of the user study session in study 1. After entering the survey, participants were first shown the two samples of self-introduction and SAMI's inferences, then prompted to answer their perceived accuracy of SAMI's inferences, the trust measurement, and the social perception measurement. The two samples were the same samples shown to the participants in study 1. We also randomized the order of the two samples being shown to the participants in the survey to remove potential order effect. Participants were then asked to enter their Prolific ID on another website to retrieve SAMI's inferences about them, and then fill out the same perception measurements. At the end of the survey, a debriefing form informing participants about the real purpose of the study and how SAMI's inferences were fabricated based on their personality survey answers were provided. Participants were compensated with \$3 USD for completing the experiment survey, and an extra \$4 USD bonus for completing both surveys. We received 211 responses (n=61 for accurate condition, n=151 for inaccurate condition) for the experiment survey. The median completion time for the experiment survey is about 12 min. 

% In our data processing of the experiment survey data, we removed ten participants' data given that they finished the experiment survey way too fast, in less than six minutes; we also removed an additional three participants' data given that there were obvious and prevalent contradictions in their survey responses. We ended up with 198 participants' data for experiment survey. 

% \subsubsection{Study 2 Measures}
% \chelsea{Study 1 Method will briefly mention the perception measures since the measures are now considered "probes."} 
% In this section, we describe the three scales that we used in the preliminary survey and the experiment survey that measured our moderator (AI literacy) and perception outcomes (trust, intelligence, anthropomorphism, and likeability). 

% \textbf{General AI Literacy Scale: } This 13-item scale was developed and validated by~\citeauthor{pinski2023ai} to measure general AI literacy, which they interpreted as ``humans' socio-technical competences regarding AI''~\cite{pinski2023ai}. This scale consists of five dimensions: AI technology knowledge, human actions in AI knowledge, AI steps knowledge, AI usage experience, and AI design experience. The responses were given to the 13 items on a five point Likert scale. Correlation test suggested that the five dimensions are highly inter-correlated, with correlation ranging from 0.31 to 0.73. To avoid inflating our model, we decided to use an overall literacy score that captures all these dimensions by taking the sum of the score for each dimension. 

% %%%%% explain the two significant moderator in post-hoc
% % This general AI literacy scale measures five dimensions of general AI literacy:~\textit{AI technology knowledge}, which measures participants' knowledge regarding what makes AI distinct from other technology and the role of AI in human-AI interaction;~\textit{Human actions in AI knowledge}, which measures participants' knowledge of the role of human actors in human-AI interaction; ~\textit{AI steps knowledge}, which measures participants' knowledge about AI's input, processing, and output and each step's impact on humans;~\textit{AI usage experience}, which measures participants' use experience with AI;~\textit{``AI design experience''}, which measures participants' experience in designing and developing AI models and/or AI-driven products. 

% % An overall AI literacy score was calculated by taking the sum of the score for each AI literacy dimension given that these dimensions are highly correlated with each other. We found these dimensions are highly inter-correlated, ranging from XX to XX. For the sake of simplicity in our model, we decided to use an overall literacy score that captures all these dimensions by taking the sum of them. \chelsea{@vedant I forgot why we decided to take the sum of all the AI lit dimensions... Was it because they were all highly correlated? And if so, how should I report the correlation here?}

% \textbf{Human-Computer Trust Scale:} We measured students' trust in SAMI by using the ``Human-Computer Trust Scale (HCTS)'' developed and validated by~\citeauthor{gulati2019design}. This scale consists of 12 statements that can be customized to the specific AI technology being studied, and responses were taken on a five-point Likert scale. This scale measures four dimensions of trust: perceived risk, benevolence, competence, and overall trust. Given that the scores for each of the dimensions were highly inter-correlated, with correlations ranging from -0.45 to 0.75, we took the score for overall trust to represent participants' trust in SAMI in our analysis. 

% % aims at measuring four dimensions of trust, and consists of 12 statements that can be customized to the AI technology studied and responses were taken on a five-point Likert scale with labels for ``Strongly Disagree'' (1), ``Neither Agree nor Disagree'' (3), ``Agree Strongly'' (5). 

% % We chose this scale given its focus on human-AI interaction and the multiple dimensions of trust it measures:~\textit{Perceived Risk, Benevolence, Competence, and Overall Trust.} ~\textit{Perceived risk} measures participants' assessment of the likelihood of certain incident happening with the use of certain technology and how concerned they would be with the consequences;~\textit{Benevolence} measures participants' perceptions of the helpfulness of the technology to help users achieve their goals;~\textit{Competence} measures participants' perception of whether the technology has all the features and functionalities to perform its intended tasks;~\textit{Overall Trust} measures participants' level of overall trust on the technology. 

% % A score for each dimension was calculated by taking the average of participants' reported score of statements that aimed at measuring the corresponding dimension. Given that the scores for each of the dimensions were highly inter-correlated (give a range OR .x with this dimension ``to avoid inflating the model'') \chelsea{@vedant how should I report the correlations here since there are multiple?}, we took the score for overall trust to represent participants' trust in SAMI in our analysis. 

% \textbf{Godspeed Scale for Human-Robot Interaction:} We measured students' social perception in SAMI by using the Godspeed scale developed and empirically validated by~\citeauthor{bartneck2009measurement}. This scale has been widely used to measure user's social perception of AI agent in prior literature (e.g.,~\cite{wang2021towards}). This scale is a semantic differential scale that asks participant to indicate their position on a scale between two bipolar words (e.g., Fake 1 2 3 4 5 Natural). Given that some of the dimension measurements are only applicable to robots (e.g., animacy and perceived safety), we adapted the scale and only took the three dimension measurements that are applicable to SAMI:~\textit{Anthropomorphism, Perceived Intelligence, and Likeability.}~\textit{Anthropomorphism} measures participants' level of attribution of human forms or human characteristics to the agent;~\textit{Perceived Intelligence} measures participants' perception of how smart or intelligent the agent is;~\textit{Likeability} measures participants' level of positive impression of the agent. A score for each dimension was calculated by taking the average of participants' reported score of statements with the corresponding dimension. 


==> source/00packages.tex <==
\usepackage{amsmath}
\usepackage{multirow}
\usepackage{pbox}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{atbegshi,picture}

\definecolor{DarkBlue}{HTML}{00008B}
\definecolor{green}{rgb}{0.0, 0.65, 0.31}
\definecolor{purple}{HTML}{ae017e}


\newif{\ifhidecomments}
  \hidecommentsfalse 
\ifhidecomments
    \newcommand{\chelsea}[1]{}
    \newcommand{\chidy}[1]{}
    \newcommand{\vedant}[1]{}
    \newcommand{\ashok}[1]{}

\else
    \newcommand{\chelsea}[1]{\textbf{\small\sffamily{\textcolor{purple}{[#1 -- Chelsea]}}}}
    \newcommand{\vedant}[1]{\textbf{\small\sffamily{\textcolor{DarkBlue}{[#1 -- Vedant]}}}}
    \newcommand{\chidy}[1]{\textbf{\small\sffamily{\textcolor{green}{[#1 -- Chidy]}}}}
    \newcommand{\ashok}[1]{\textbf{\small\sffamily{\textcolor{red}{[#1 -- Ashok]}}}}
  \fi
\newcommand{\edit}[1]{{\textcolor{editCol}{#1}}}
\newcommand{\mask}[1]{{\textcolor{maskCol}{#1}}}

==> source/1introduction.tex <==
\section{Introduction}
Recently, a plethora of hyper-personalized AI systems that can profile users' characteristics and traits have been deployed in people's daily lives, with the ultimate goal of providing personalized shopping, music, and social media recommendations. As these systems become more advanced in profiling people's most personal and complex traits such as personalities and emotions~\cite{hall2017say,gou2014knowme,liao2021crystal}, they sometimes give people the illusion that ``machines can read our minds''~\cite{guzman2020ontological}. This illusion has led to various---rather concerning---reactions and perceptions of AI with people attributing AI with beyond-human expertise at reading people's emotions and personalities~\cite{warshaw2015can,hollis2018being}. However, people's perceptions and reactions of AI when this illusion is broken in the face of~\textit{AI misrepresentations} have not yet been explored. 

% \chelsea{need to talk about AI literacy and AI knowledge in Intro}
% While many heuristics and theories have been proposed to explain such perceptions and attitudes towards AI, such as machine heuristic~\cite{sundar2019machine,sundar2020rise} and the Computers are Social Actors (CASA) paradigm~\cite{nass1994computers}, existing theories and empirical studies have not studied users' perceptions and reactions in the face of AI misrepresentations.


% Recently, a plethora of hyper-personalized systems powered by AI algorithms that can profile users' characteristics and traits (e.g., personality traits) have been developed and used in people's daily lives, with the ultimate goal of providing personalized recommendations across areas such as shopping, music recommendations, and social media feeds. As these systems become more advanced~\cite{hall2017say,gou2014knowme,liao2021crystal}, they sometimes give people the illusion that ``machines can understand us and read our minds''~\cite{guzman2020ontological}. This illusion has led people to various---rather concerning---reactions and perceptions of AI when interacting with hyper-personalized systems: people considered AI-generated personality profiles to be ``creepily accurate''~\cite{gou2014knowme,warshaw2015can,liao2021crystal,kim2020understanding}, attributing AI with beyond-human expertise of reading people's emotions and personalities~\cite{warshaw2015can,hollis2018being}, and believing that AI could identify their ``hidden self'' that they weren't aware of themselves~\cite{hollis2018being}. 

% Many heuristics and theories have been proposed to explain and understand people's perceptions and attitudes towards AI. For example, people's tendency to ascribe more trustworthiness to AI than humans has been largely explained by machine hueristic~\cite{sundar2019machine,sundar2020rise}, a rule of thumb that people believe machines are logical, objective, and emotionless, and hence more trustworthy than humans; people's social responses and attitudes towards AI has been interpreted using the Computers Are Social Actors (CASA) paradigm~\cite{nass1994computers}. Much of prior work has also looked into people's various folk theories~\cite{devito2017platforms,liao2021crystal} and mental models~\cite{gero2020mental,wang2021towards} of AI systems to understand people's sense-making process of AI, hoping to explain people's emotional and logical responses to AI systems. 


AI misrepresentations is one type of AI fallibilities when AI misinterprets people's most intimate and complex traits like personality and emotions, aspects where people possess the most self-awareness. Prior work has suggested that AI mistakes on human-AI tasks could erode people's trust and social perceptions (e.g., anthropomorphism, intelligence, likeability) of the AI~\cite{honig2018understanding,salem2015would}. However, when faced with AI misrepresentations of people's most intimate traits, people may dismiss it based on their self-awareness, resulting in lack of adherence and trust in AI; or people might exhibit unwavering trust in AI, allowing it to persuade them into accepting false information about themselves. 

% AI misrepresentations are AI fallibilities in interpreting people's most intimate characteristics such as personality traits and emotions--- aspects where people possess the most self-awareness. Prior work has suggested that AI mistakes could erode people's trust and social perceptions of the AI~\cite{honig2018understanding,salem2015would}. However, when faced with AI misrepresentations of their most intimate traits, people may promptly dismiss it based on their self-awareness, or they might exhibit unwavering trust in AI, allowing the technology to persuade them into accepting inaccurate inferences about themselves. 


% Even algorithms with supposedly high accuracy can make mistakes when powering hyper-personalized AI systems in-the-wild~\cite{rao2015they}. 
% % However, existing studies and theories to understand people's reactions and perceptions of hyper-personalized AI systems have not specifically focused on the scenario where the AI misinterpreted people's characteristics and traits, which could lead the AI to misrepresent people within human communities. 
% While prior work has suggested that AI mistakes could have a negative impact on people's trust and social perceptions of AI~\cite{honig2018understanding,salem2015would}, AI misrepresentations are AI mistakes in interpreting people's most personal and implicit characteristics such as personality traits and emotions, which people themselves are supposedly to know the most about. When confronted with AI misrepresentations, it could be that people would immediately dismiss it given their understandings about themselves; or people's over-trust in AI persisted so much that they were persuaded by the AI into believing inaccurate inferences about them. 

Even algorithms with supposedly high accuracy can make mistakes when powering hyper-personalized AI systems in-the-wild~\cite{rao2015they}. Understanding people's reactions and perceptions of the AI after encountering AI misrepresentations could offer valuable insights into whether and how people changed their intuitions, beliefs, and reactions of AI in the face of AI fallibilities. This could provide critical implications for the future design and development of responsible interventions, mitigation, and repair strategies to retain user trust, minimize harms, and prevent overreliance when such AI systems inevitably err. In this paper, we seek to understand people's reactions and perceptions of AI after encountering personality misrepresentations by AI. We contextualized this research aim in higher education given the increasing use of hyper-personalized AI systems to identify student characteristics and traits, especially personality traits, to facilitate school project team formations~\cite{xiao2019should,alberola2016artificial,jahanbakhsh2017you,lykourentzou2016personality}. Specifically, this paper explores three research questions:


% investigate these questions in the context of personality-based AI-facilitated team matching in education context given the increasing use of AI systems that could identify personality to help facilitate school project teams. We took a mixed-methods approach and conducted two studies to explore this problem space: we first qualitatively explored students’ reactions and sense-making process of seeing AI-generated personality profiles of them; we then conducted a large-scale survey study to quantitatively explore the effect of AI’s profiling mistakes on students’ perception of AI and further explored factors that could mediate changes in user perceptions of AI after encountering profiling mistakes. 

\begin{table}[h]
% \sffamily
\centering
% \footnotesize
\vspace{-0.5em}
\begin{tabular}{@{}l@{}p{0.92\columnwidth}@{}}
    \textbf{RQ 1: } & What perceptions and reactions do students have about the AI after encountering AI misrepresentations of their personality traits in AI-facilitated team matching?\\
    \textbf{RQ 2: } & How do students change their perceptions of the AI after encountering AI misrepresentations of their personality traits in AI-facilitated team matching? \\
    \textbf{RQ 3: } & What factors contribute to students' perception changes after encountering AI misrepresentations of their personality traits in AI-facilitated team matching? \newline 
    % \begin{tabular}{@{}l@{}p{0.85\columnwidth}@{}}
    % \textit{RQ 3.1: } & What is the effect of AI misrepresentation on students' overall trust and social perceptions of the AI?  \\
    % \textit{RQ 3.2: } & How does students' levels of general AI literacy moderate the effect of changes in students' perception of AI after encountering AI misrepresentation? \\
    % \end{tabular}
    % \bottomrule
\end{tabular}
\vspace{-0.9em}  
\end{table}

\vspace{-0.7em}
To answer these research questions, we conducted semi-structured interviews with twenty college students (Study 1) and a large survey experiment (Study 2) with 198 students on the Prolific platform. In both studies, we took a Wizard-of-Oz approach to fabricate intentionally inaccurate/accurate personality inferences based on participants' personality ground truth. We showed participants in both studies their ``AI-generated personality inferences'' to elicit their perceptions and reactions of AI misrepresentations. We found that people's existing and newly acquired AI knowledge plays a critical role in shaping their perceptions and reactions after encountering AI misrepresentations. Specifically, we pinpointed three rationales that people adopted through knowledge acquired from AI (mis)representations: AI works like a machine, human, and/or magic. These rationales are highly connected to their reactions of over-trusting, rationalizing, and forgiving of AI misrepresentations. We also found that people's existing AI knowledge, i.e., AI literacy, significantly moderate the level of changes in people's overall trust after encountering AI misrepresentations. 

% Through our analysis, we pinpointed three rationales that people employed when interpreting the AI: AI works like a machine, AI works like a human, AI works like magic. We found that people over-trusted and rationalized AI misrepresentations, expressed concerns and/or lack of concerns about AI misrepresentations, all of which could be explained by the specific rationale they were employing at the time. We also found that encountering AI misrepresentations significantly lowered people's overall trust, perceived intelligence, anthropomorphism, and likeability of the AI, with AI literacy as a significant moderator on the level of changes in people's overall trust. 

% Based on our findings, we discussed using the three rationales as a unifying lens to explain and understand people's reactions and perceptions of AI after encountering AI misrepresentations. We then outlined implications for future design and development of ethical and resilient rationale-based AI recovery strategies. 

The contribution of our work is three-fold. First, we highlight the role of people's existing and newly acquired AI knowledge in shaping their perceptions and reactions to AI after encountering AI misrepresentations. Second, we provide a descriptive account of people's re-framing of their perceptions through adopting various rationales in the face of AI misrepresentations.
% how people's newly acquired knowledge of AI can lead to a re-framing of their perceptions, i.e., adopting various rationales, in the face of AI misrepresentations.
% people's perception changes in the face of AI misrepresentations through rationales. 
We connect this process to people's reactions of over-trusting, rationalizing, and forgiving of AI misrepresentations. Finally, we provide a set of implications and future directions for the design and development of intervention, mitigation, and repair strategies to consider people's AI knowledge to reduce potential harm. 

% provide a descriptive account of people's process of perceptions changes in the face of AI misrepresentations through rationales. 

% we identified three rationales and proposed it as a unifying lens to explain and understand people's reactions and perceptions of AI after encountering AI misrepresentations. Second, we offered empirical evidence on how people's perceptions changed after encountering AI misrepresentations, highlighting the role of AI literacy in moderating the effect of AI misrepresentations in changes in overall trust. Finally, we provided a set of implications and future directions for the design and development of ethical and resilient hyper-personalized AI systems. 




==> source/2relatedwork.tex <==
\section{Related Work}

\subsection{People's Perceptions and Reactions of Hyper-Personalized AI}
Much HCI work has been conducted to understand people's reactions and concerns to hyper-personalized AI systems that can profile people's emotions~\cite{wang2020sensing,disalvo2022reading,hollis2018being} and personality characteristics~\cite{gou2014knowme,warshaw2015can,liao2021crystal,volkel2020trick}. Prior work found that most people perceived their AI-generated personality profiles to be ``creepily accurate''~\cite{gou2014knowme,warshaw2015can,liao2021crystal,kim2020understanding}. Other studies demonstrated people's tendency to over-trust AI-generated personality profiles about them. Studies showed that people felt unqualified to modify their personality profile generated by the ``expert'' algorithm~\cite{warshaw2015can}, sometimes even overriding their own personal judgments about themselves due to the belief that the AI algorithm could identify their ``hidden self'' and had privileged information about them~\cite{hollis2018being}.

% Other studies showed people's tendency to over-trust AI, even though AI-generated personality profiles were about the users themselves:~\citeauthor{warshaw2015can} [2015] found that people felt unqualified to modify their personality profile generated by automated personality recognition algorithm due to their over-trust in the ``expert'' algorithm;~\citeauthor{hollis2018being} [2018] echoed this finding and added further that some users even overrode their personal judgements about their emotions, and believed that the AI algorithm was capable of identifying their ``hidden self'' and had privileged information about their emotions. 

% There is also a growing body of research in HCI focused on studying people's reactions and attitudes of towards AI algorithms such as recommendation algorithms, with ``trust'' as the core concept of interest. Much research in this area suggested that people had a tendency to overtrust AI~\cite{oh2022you,banas2022machine,kapania2022because} and to attribute more credibility to AI~\cite{kapania2022because,edwards2016robots} comparing to human agents--- some even pointed out that AI was considered as an authority figure that could influence people's behaviors without needing to provide adequate evidence~\cite{kapania2022because}. In their interview study on people's perceptions and attitudes of AI in India,~\citeauthor{kapania2022because} [2022] found that people seemed to have a high tolerence of AI failures, with some displaying tendencies of forgiving and justifying AI misfires, or even blame themselves or others for AI's mishaps~\cite{kapania2022because}. Many researchers attributed this tendency to overtrust AI to people's machine heuristics~\cite{sundar2020rise}: the belief that machines are objective, emotionless, and logical entities without feelings, therefore more trustworthy comparing to humans~\cite{sundar2020rise}.  

% Despite people's tendency to trust AI-generated information about them, people largely remained cautious about sharing it with others to carefully maintain their self-presentations through AI-facilitated channels. Many users of automated personality recognition AI were concerned about the implications of sharing or not sharing their personality profiles: some users wanted control over modifying their profile and traits before sharing due to concerns over others' misinterpretations of AI-inferred traits about them~\cite{gou2014knowme}; however, others felt compelled to share despite their reservations about sharing given that, in their opinions, not sharing would be indicative of them having something to hide~\cite{warshaw2015can}. Since our interactions and communications with each other are heavily mediated through AI~\cite{hancock2020ai} nowadays, people perceive themselves~\cite{devito2017platforms,karizat2021algorithmic}, others~\cite{eslami2015always,jakesch2019ai}, as well as their relationships with others~\cite{eslami2015always,eslami2016first,mieczkowski2021ai} through AI-filtered lens. Prior work in AI-mediated communication suggested that self-presentations or impressions, when knowingly augmented by AI, can decrease its perceived trustworthiness~\cite{jakesch2019ai} and undermine social attractions between people~\cite{mieczkowski2021ai}.~\citeauthor{eslami2015always} found that people formed misperceptions about their Facebook friends whose posts never showed up on their feed due to lack of understanding of the recommendation algorithm, which led them to make false inferences about their relationships with that person. 

% Many heuristics and theories have been proposed to explain and understand people's perceptions and attitudes towards AI. For example, people's tendency to ascribe more trustworthiness to AI than humans has been largely explained by machine hueristic~\cite{sundar2019machine,sundar2020rise}, a rule of thumb that people believe machines are logical, objective, and emotionless, and hence more trustworthy than humans; people's social responses and attitudes towards AI has been interpreted using the Computers Are Social Actors (CASA) paradigm~\cite{nass1994computers}. Much of prior work has also looked into people's various folk theories~\cite{devito2017platforms,liao2021crystal} and mental models~\cite{gero2020mental,wang2021towards} of AI systems to understand people's sense-making process of AI, hoping to explain people's emotional and logical responses to AI systems. 

Scholars have developed many theories to explain people's reactions and perceptions of AI systems~\cite{sundar2019machine,sundar2020rise,devito2017platforms,nass1994computers,guzman2020ontological}. Theories such as Machine Heuristic, a rule of thumb that people believe machines are logical, objective, and emotionless, and hence more trustworthy than humans, has been used to explain people's tendency to over-trust AI outcomes~\cite{oh2022you,banas2022machine,kapania2022because,edwards2016robots}; the Computers Are Social Actors (CASA) paradigm has been used to explain people's social reactions to forgive, tolerate, and justify AI misfires~\cite{nass1994computers,kapania2022because}; learning science theories such as conceptual changes~\cite{ozdemir2007overview} and ontological shift~\cite{slotta2011defense,chi1994things} have also been used to examine how people conceptualize the ontological differences between humans and computers~\cite{guzman2020ontological}. Together, these theories suggest people's increasingly blurred conceptualizations and reactions between machines and humans due to technologies' human-like behaviors and capabilities~\cite{guzman2020ontological}. 

Empirical studies in HCI have examined people's various folk theories~\cite{devito2017platforms,liao2021crystal}, mental models~\cite{gero2020mental,wang2021towards}, and factors that influence these perceptions of AI systems. Scholars have found that people with limited folk theories about the data source, data scope, and personalization of the AI algorithm tend to dismiss AI's personality inferences as less threatening~\cite{liao2021crystal}. Additionally, factors such as the data-driven aspect of the system, the ambiguity around how the system works could all influence people's trust and perceptions of the result of AI-generated personality inferences~\cite{kim2020understanding}. Research has also found that people's AI literacy~\cite{druga2017hey,long2020ai,shin2022people,schoeffer2022there} and personal investment in the AI's output~\cite{eslami2019user} play a crucial role in shaping their perceptions, especially trust, in the AI systems. This suggests that people's pre-existing and evolving knowledge about AI could be critical in their perceptions of the AI, which has been under-explored. 

\subsection{Responding and Mitigating AI Fallibilities} Although much work in human-robot interaction has examined people's perceptions of AI agents after encountering AI failures, these studies suggest mixed results. On the one hand, prior work showed that encountering robot failures would significantly lower people's perceptions of the robot~\cite{honig2018understanding} in terms of robots' trustworthiness~\cite{salem2015would,law2017wizard,roesler2020effect,hsu2021attitudes}, perceived intelligence~\cite{takayama2011expressing}, perceived likeability~\cite{mirnig2017err}, anthropomorphism~\cite{salem2015would}, reliability~\cite{salem2015would}, and ease of use~\cite{de2023we}. On the other hand, other research has suggested that AI mistakes could be considered as human-like characteristics, and therefore making the interactions more engaging~\cite{honig2018understanding,law2017wizard} and pleasurable~\cite{mirnig2017err,honig2018understanding,gompei2015robot}, mitigating the potential negative effect AI mistakes might have on users' perceptions of the AI~\cite{honig2018understanding,buhrke2021making,mirnig2017err}. 
% For instance,~\citeauthor{mirnig2017err} [2017] did not find a significant difference in perceived intelligence and anthropomorphism between participants who interacted with faulty robots vs. flawless robots~\cite{mirnig2017err}; studies also suggested that robot failures might make users' interaction experience more pleasurable~\cite{mirnig2017err,honig2018understanding,gompei2015robot} and more engaged~\cite{honig2018understanding,law2017wizard}. 
Scholars conjectured that people's perception after encountering robot failures might be attributed to various factors such as types of failures, failure severity, or the nature of the task (e.g., formal workplace or social and personal)~\cite{sarkar2017effects,honig2018understanding,rossi2017timing}. Examining people's perception changes after encountering AI mistakes across contexts could better inform the design of AI's repair and recovery strategies. 

Following this line of research, others investigated AI's repair and mitigation strategies, focusing mostly on conversation breakdown during human-chatbot interactions~\cite{ashktorab2019resilient,mahmood2022owning} and human-robot interactions~\cite{honig2018understanding}.~\citeauthor{honig2018understanding} [2018] provided a comprehensive summary of four types of mitigation strategies during interaction breakdowns: (1) Setting expectations by forewarning users about potential flaws~\cite{lee2010gracefully,honig2018understanding,kocielnik2019will}, (2) Communicating errors properly by incorporating elements such as apologizing~\cite{mahmood2022owning}, humor~\cite{clausen2023exploring}, or through further explanations~\cite{ashktorab2019resilient}, (3) Asking users for help, and (4) Mix and match of different mitigation strategies listed above. One particular mitigation strategy that has gained popularity is explainable AI. However, empirical studies have suggested that common explanation strategies were not as effective as expected given that the explanations did not take into account people's domain expertise~\cite{wang2021explanations} and AI knowledge such as intuitions and beliefs~\cite{chen2023understanding}. This has sparked the area of human-centered explainable AI~\cite{miller2019explanation,liao2021human,ehsan2020human} that aims at presenting explanations relative to people's knowledge, capabilities, and beliefs.

% However, only a few work has empirically studied people's reactions and attitudes towards AI mistakes, and suggested additional, sometimes contradictory findings. For example, instead of overtly positive view and reliance on AI,~\citeauthor{hsu2021attitudes} [2021] found that students perceived AI autograders as unfair and harmful due to their over-estimation of the AI's error rate~\cite{hsu2021attitudes}. While~\citeauthor{oh2022you} [2022] corroborated with findings from prior literature that people tended to have greater trust and more positive attitudes towards machine-generated recommendations comparing to human-generated recommendations, they also found that people's trust and general attitudes declined quickly after users saw machines made mistakes (also known as the phenomenon of algorithm aversion~\cite{dietvorst2015algorithm}). This suggested that multiple heuristics could exist and interact together to shape people's perceptions and attitudes towards AI after encountering AI mistakes. 

% \chelsea{need to add a paragraph about AI repair and explanation and transparency here. }

% \cite{honig2018understanding}: mitigation strategies: 
% - setting expectations (giving the user advanced notice regarding potential failures): setting expectations by forewarning improved evaluation of the robot and judgements of the quality of the service.  \cite{lee2010gracefully}
% - communicating properly: politeness strategies, apologizing~\cite{mahmood2022owning}, expressing regret, humor~\cite{clausen2023exploring}. Explanation, paraphrasing, simplifying language
% - asking users for help: 
% - mix and match: 

% \cite{miller2019explanation}: explanations are conrastive, selected and social. selected: Humans are adept at selecting one or two causes to be the explanation, cognitive bias; Social: Explanations are a transfer of knowledge, presented relative to the explainer's belifs about the explainee's beliefs

% \cite{ehsan2020human}: turn to the sociotechnical: perception differences due to users' backgrounds. Explanations, by definition, are context-sensitive. 

% \cite{liao2021human}: theories of human cognition and behaviors can offer conceptual tools to inspire new computational and design frameworks for XAI. 

% \cite{ashktorab2019resilient}: We found that providing options and explanations were generally favored, as they manifest initiative from the chatbot and are actionable to recover from breakdowns. Preferences for repair strategies are not universal. Acknowledging misunderstanding with forthrightness and less redundancy. Intelligent repair with user control. 

% \cite{sharifheravi2020sa}: significant effect of transparency on trustworthiness. transparency was most beneficial for trust repair following the disaster. participants perceived the high-anthropomorphic AI to be less competent and less trustworthy than the low anthropomorphic AI. 

% \cite{wang2021explanations}: the effects of AI explanations are largely different on decision making tasks where people have varying levels of domain expertise in, and many AI explanations do not satisfy any of the desirable properties for tasks that people have little domain expertise in. 

% \cite{chen2023understanding}: While many factors may affect reliance on AI support, one important factor is how decision-makers reconcile their own intuition—beliefs or heuristics, based on prior knowledge, experience, or pattern recognition, used to make judgments—with the information provided by the AI system to determine when to override AI predictions. Our results identify three types of intuition involved in reasoning about AI predictions and explanations: intuition about the task outcome, features, and AI limitations. Building on these, we summarize three observed pathways for decision-makers to apply their own intuition and override AI predictions.







==> source/3studyoverview.tex <==
\section{Study Overview}
\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{source/figures/study_procedure.pdf}
    \caption{Study flow diagram that shows the procedures of Study 1 and Study 2. Study 2 occurred after Study 1 was concluded. All personal inferences shown to participants were either accurate or inaccurate based on the condition assigned to the participants.}
    \label{fig:study_procedure}
\end{figure}

To examine people's reactions and perceptions of AI after encountering AI misrepresentations, we conducted two studies using a mixed-methods approach. The first study (Study 1) focuses on qualitatively exploring students' perceptions and reactions to AI after encountering AI misrepresentations, and the second study (Study 2) focuses on quantitatively examining the factors, specifically AI literacy, contributed to the variations in students' perceptions of the AI after encountering AI misrepresentations. Given that AI output is often non-deterministic and thus difficult to control and manipulate, we took a Wizard-of-Oz approach to fabricate and control the accuracy of the AI inferences--- in both studies, human researchers fabricated all the AI inferences based on participants' personality ground truth, collected in the preliminary survey in each study. To prevent raising participants' suspicions when shown fabricated AI inferences, they were not presented with the inferences until at least a week after they completed the preliminary survey. 

To compare and contrast participants' reactions and perceptions of AI misrepresentations, we divided all participants into two conditions in both studies: participants in the accurate condition received accurate ``AI inferences,'' and the inaccurate condition received inaccurate ``AI inferences.'' In both studies, participants were asked to evaluate AI-generated inferences based on students' self-introduction paragraphs, which will be used by an AI agent named SAMI (stands for ``Social Agent Mediated Interaction'') to match them with potential teammates for a school project. 

% These inferences will be leveraged to help match the student to other potential teammates for a school project. However, due to the constraints of the study, participants were only asked to evaluate SAMI's inferences about them during the studies.

In Study 1, we conducted user study sessions to understand students' reactions and perceptions (RQ1, RQ2) of the AI after encountering AI (mis)representations by showing them different SAMI inferences, including inferences about themselves. Based on our observations in Study 1, we revised some of the measurements and replicated Study 1 as a survey experiment without the semi-structured interview part. We conducted Study 2 on the Prolific crowdsourcing platform to obtain a larger sample to examine changes in students' perceptions (RQ2) and factors that contributed to those changes (RQ3). Both studies were approved by the IRB at the researchers' institute. Before Study 1, we conducted a pilot study with 14 people to test out the study procedure and the SAMI inference fabrication process. 


==> source/4study1.tex <==
\section{Study 1: Understanding Students' Perceptions and Reactions to AI Misrepresentation}
In this section, we first describe the method we used in Study 1, including recruitment, study setup, and study procedure. We then talk about our data analysis process. Finally, we present our findings on students' perceptions and reactions to SAMI misrepresentations. 

\subsection{Study 1 Method}
\subsubsection{Study 1 Participant and Recruitment}
We conducted remote 60-minute user study sessions with 20 current students, all recruited from a large public U.S. technology institute. We recruited our participants by posting our recruitment message on the institute's Reddit and by broadcasting our recruitment email to different departments and programs, especially non-STEM programs, within the institute to increase sample diversity. Our recruitment message invited students to evaluate an AI agent SAMI that could perform team matching by drawing inferences from students’ self-introduction. Students signed up for the study by filling out a preliminary survey.

In the preliminary survey (see Supplementary Materials~\ref{supp:s1_prelim_survey}), students wrote a paragraph of self-introduction as a free-flowing essay to introduce themselves to SAMI. They then completed a 44-item Big Five personality survey measurement to provide ground truth of their personality. 
% We chose the 44-item personality scale because it provides us with sufficient personality statements to facilitate our inference fabrication process (details in Section~\ref{fabrication}). 
Students were then asked about level of technology proficiency (``Beginner'', ``Intermediate'', or ``Expert.''), general attitude towards AI technology on a scale of ``1-Very negative'' to ``5-Very positive'', as well as their demographic information, level of study, major, academic or professional background. 

We received 110 valid preliminary survey responses. We sent out follow-up invitations in batches to balance sample diversity and ended up with 20 participants in total. We then evenly assigned these participants to either the inaccurate or accurate condition (10 participants in each condition) while balancing the sample diversity in each condition. The median age of our participants was 20 years old. There were 15 undergraduate students and 5 master's students in our study. Their gender breakdown is as follows: women (n=10), men (n=7), non-binary (n=2), one participant did not report their gender. Our participants came from a variety of majors, with mostly intermediate tech proficiency, and varying general attitudes toward AI. Table~\ref{tab:s1_participant} in Appendix~\ref{appendix:s1participant} shows the information for all the participants in Study 1.


% We then proceeded with inference fabrication for these participants, which we describe next. 

% The median age of our participants was 20 years old. There were 15 undergraduate students and 5 master students in our study. Their gender breakdown is as follows: women (n=10), men (n=7), non-binary (n=2), one participant did not report their gender. Our participants came from a variety of majors, with mostly intermediate tech proficiency, and varying general attitudes toward AI. Table~\ref{tab:s1_participant} shows the information for all the participants in study 1. All 20 participants were compensated with \$25 gift card each for their time. 

% \begin{table}[]
%     \centering
%     \small
%     \footnotesize
%     \caption{Study 1 participant information. In the Gender column, ``W'' stands for ``Woman'', ``M'' stands for ``Man'', ``NB'' stands for ``Non-Binary.'' In the Level of Study column, ``UG'' stands for ``Undergraduate.'' In the Major column, ``Eng.'' stands for ``Engineering'', ``Comp.'' stands for ``Computational.'' In the Tech Proficiency column, participants self-reported their technology proficiency as ``Beginner'', ``Intermediate'' or ``Expert.'' In the Attitudes Toward AI column, participants self-reported their attitudes toward AI on a scale of ``1-Very Negative'' to ``5-Very Positive.''}
%     \begin{tabular}{clllllll} \toprule
%     % \begin{tabular}{M{3cm}|M{1.5cm}|M{1.5cm}|M{1.5cm}|M{2cm}|M{4.5cm}|}
%      \textbf{Condition} & \textbf{ID} & \textbf{Age}  &   \textbf{Gender}  &   \pbox{1cm}{\textbf{Study \newline Level}}  &   \textbf{Major} & \pbox{2cm}{\textbf{Tech \newline Proficiency}}     &       \pbox{3cm}{\textbf{Attitudes \newline Toward AI}}\\ \midrule
%      \multirow{10}{5em}{\centering Accurate Condition (n=10)} &   P14    &  22     &    W    &    UG    &    Psychology     &       Intermediate    &   Neutral to Positive \\
%                & P19  &  18    &   W   &    UG    &    Psychology    &    Intermediate      &       Neutral to Negative \\
%                & P22  &  28    &   W   &    Master    &    Digital Media    &    Intermediate       &       Neutral \\ 
%                & P26  & 21      & M     & Master    & Digital Media     & Intermediate      &   Neutral \\
%                & P29    & 19    & W     &   UG      & Neuroscience      & Intermediate  & Neutral to Negative \\
%                & P30    & 31    & W     &   Master     & HCI      & Expert  & Neutral to Positive \\
%                & P33    & 19    & M     &   UG     & Chemical Eng.      & Intermediate  & Neutral to Positive \\
%                & P34    & 19    & NB     &   UG     & Comp. Media      & Intermediate  & Very Positive \\
%                & P37    & 20    & M     &   UG     & CS      & Expert  & Very Positive \\
%                & P40    & 19    & M     &   UG     & Computer Eng.     & Intermediate  & Very Positive \\   \midrule
%     \multirow{10}{5em}{\centering Inaccurate Condition (n=10)} & P16    &   19  & W     &   UG  &   Psychology  &   Intermediate    &   Neutral to Positive \\
%     & P17  &  21    &   W   &    UG    &    Psychology    &    Intermediate      &       Neutral \\
%     & P21  &  19    &   NB   &    UG    &    Psychology    &    Expert      &       Neutral to Positive \\
%     & P23  &  20    &   W   &    UG    &    Psychology    &    Intermediate      &       Neutral to Negative \\
%     & P24  &  23    &   W   &    Master    &    HCI    &    Intermediate      &       Neutral to Positive \\
%     & P28  &  20    &   W   &    UG    &    Business Admin    &    Intermediate      &       Neutral to Positive \\
%     & P35  &  22    &   M   &    Master    &    CS    &    Expert      &       Neutral to Positive \\
%     & P36  &  22    &   M   &    UG    &    Industrial Eng.    &    Expert      &       Neutral \\
%     & P39  &  21    &   No report   &    UG    &    Biology    &    Intermediate      &       Neutral to Positive \\
%     & P41  &  18    &   M   &    UG    &    Computer Eng.    &    Expert      &       Neutral to Positive \\
%     \bottomrule
       
%     \end{tabular}
    
%     \label{tab:s1_participant}
% \end{table}

\subsubsection{Fabricating SAMI Inferences} \label{fabrication}

% \begin{figure}
%     \centering
%     \includegraphics[width=\textwidth]{source/figures/fabrication.pdf}
%     \caption{This figure shows the sample and our inference fabrication process for the sample student. The top half of this figure shows one of the samples we showed to the participants that is inaccurate. The bottom half of this figure shows how we utilized participant's personality ground truth filled out in the preliminary survey to fabricate inferences for them based on the condition they were assigned to.}
%     \label{fig:fabrication}
% \end{figure}

We took a Wizard of Oz approach and let human researchers fabricate SAMI's personality inferences to control for inference accuracy. The fabrication of SAMI inferences was based on (1) participants' ratings of each statement on the Big Five personality test, and (2) the condition (either accurate or inaccurate) the participant was assigned to. Participants in the accurate condition would receive accurate inferences, which would consist of all the statements they rated as ``4-agree'' or ``5-strongly agree'' in the personality test, or the reverse of the statements they rated as ``1-strongly disagree'' or ``2-disagree'' in the personality test; Participants in the inaccurate condition would receive inaccurate inferences, which would consist of all the statements they rated as ``1-strongly disagree'' or ``2-disagree'' in the personality test, or the reverse of statements that they rated as “4-agree” or “5-strongly agree” in the personality test. We illustrated this fabrication process in Fig.~\ref{fig:fabrication} in Appendix~\ref{appendix:fabrication}.

When selecting statements from the personality test, we picked the three dimensions with the most extreme scores, while excluding dimensions with a neutral score of three out of five. We also restricted the length of SAMI's inferences for each participant to about 10 statements to remove the potential effect of inference length on participants' perception of SAMI. In the Big Five personality test, some statements were inherently positive and some statements were inherently negative. To remove the potential effect of the sentiment of SAMI inferences on students' perceptions and reactions to SAMI, we composed each SAMI inference with about 40\% negative inference and 60\% positive inference. 

We composed an inference fabrication guideline to document these rules and procedures (see Supplementary Materials~\ref{supp:fabrication_rule}) and closely followed the guideline when fabricating SAMI inferences.
% The fabrication guideline can be found in \chelsea{supplementary}


\subsubsection{Study 1 Remote User Study Session} 
% There are two parts in each study. In the first part of each study, we recruited potential participants by asking them to fill out a preliminary survey. In the preliminary survey, we introduced the study's goal and motivation as evaluating the performance of an AI agent and understanding their perception of an AI agent that can make inferences about them based on their self-introduction for team-matching purposes. The survey then asked them to write a short paragraph to introduce themselves to SAMI, the AI agent. Participants then filled out the Big Five personality test and answered other questions about their attitudes towards AI in general, AI proficiency/literacy, as well as demographics. Participants whose self-introductions were shorter than five full sentences were not invited to participate in the second part of the study. This requirement was implemented to make SAMI's inferences more believable to the students given the assumption that more than five full sentences there were the bare minimum of the amount of information that the AI needed to generate inferences about the student. 

% Each participant's user study session was scheduled at least a week after they filled out the preliminary survey in the hope that participants would forgot they provided their personailty ground truth information during the preliminary survey, and therefore wouldn't be suspicious of whether SAMI's inferences were generated by AI or human. 

We began each session by emphasizing to the participants that they should share their honest opinions, both positive and negative. 
% At the beginning of each session, we emphasized to each participant that they should feel free to share their honest opinions, no matter it's positive or negative. This was to avoid the possibility of participants in the inaccurate condition feeling embarrassed to express negative feelings about SAMI. 
Each study session had two parts. In the first part, participant was shown two samples of self-introductions and SAMI's inferences, then asked to fill out perception measurements (see Supplementary Materials~\ref{supp:s1_exp_survey}) to record their baseline perceptions of SAMI in terms of trust~\cite{gulati2019design} and social perceptions (likeability, perceived intelligence, anthropomorphism)~\cite{bartneck2009measurement}. Participant was then shown their own self-introduction and SAMI's inferences about them, then asked to fill out the same measurements. The goal was to record students' perceptions of SAMI immediately after each SAMI inference was presented to them. The two samples (see Supplementary Materials~\ref{supp:s1_protocol}) were written by real students from our pilot study. SAMI's inferences about the sample students were fabricated in the same way as described in section~\ref{fabrication}. SAMI's inferences for one of the samples were generated to be inaccurate, and the other one accurate. 
% An example of the sample self-introduction and SAMI's inference that was inaccurate was shown in Fig.~\ref{fig:fabrication}. 
The samples were shown in random orders to remove potential order effects. 
% This was done to give participants an idea of what SAMI's inferences looked like without biasing their perceptions of SAMI's inference accuracy. 

The second part of the session was a semi-structured interview to go through participants' reactions and perceptions of SAMI after encountering AI (mis)representations. During the interviews, we asked participants to walk us through their reactions to each of the SAMI inference, what they thought about SAMI after seeing each inference, and how they thought SAMI extracted the inferences. Throughout the interview, we used the perception measurements as a probe to provide basis for them to elaborate on their perceptions of SAMI after seeing each inference. We then debriefed the participants about the fabrication process of SAMI's inferences. We addressed any comments and questions that participants had and then provided compensation of USD \$25 gift card. All the study sessions were conducted remotely on Zoom and all lasted around 60 minutes. The session and interview protocol is attached in Supplementary Materials~\ref{supp:s1_protocol}.
% Participants took about 12 to 25 min for the first part of the session, and about 38 to 52 min for the second part of the session. 
% All the sessions were concluded at roughly the 60 min mark. We included the protocol for the user study session in supplementary materials. 

\subsection{Study 1 Data Analysis}
All sessions were video recorded and transcribed for data analysis. We adopted~\citeauthor{braun2006using}[2006]'s Reflexive Thematic Analysis (RTA) approach~\cite{braun2006using,braun2019reflecting} in our analysis. RTA encourages researchers to embrace their stance and assumptions during analysis. This differs from other qualitative data analysis approaches such as grounded theory and codebook approach that value objectivity and removing researcher bias, which does not allow enough flexibility for researchers to actively participate in the data analysis process.

Two researchers participated in the analysis to collaboratively discuss and iterate on themes that emerged from the data using RTA approach. We followed the analysis process outlined in~\citeauthor{braun2006using}[2006]. We generated our initial codes in two rounds by first dividing the 20 transcripts among the two researchers for independent coding, then swapped the transcripts for a second round of independent coding. After the initial codes were generated, the two researchers frequently met to discuss, review, and search for themes. The first round of analysis generated 16 domain categories (e.g., folk theories of SAMI) and 163 codes (e.g., believing SAMI's misrepresentation). By comparing our second round codes with the first round codes and domain categories, we distilled five themes (e.g., tendency to overtrust AI) and 27 codes (e.g., attributing human inference-making process to SAMI). We continued to review and search for larger themes and ended up distilling two bigger themes to understand students' perceptions and reactions to SAMI after encountering AI misrepresentations, which we present in detail in the next section. 

% Analyzing the interview data from the user study sessions helped shed light on students’ reaction (RQ1) and understanding of AI’s inferences (RQ2). We also used the perception measurement data in study 1 and conducted statistical analysis to offer preliminary understanding of RQ3, which helped inform the design of study 2. 

% \subsubsection{Quantitative Data Analysis}
% During the remote study sessions, we collected students' perception of SAMI in terms of trust and social perceptions before and after they encounter AI (mis)representation. Based on this data from study 1 (n=20), we conducted a preliminary exploration to examine whether encountering AI misrepresentation influenced students' perception of SAMI (RQ3.1). Prior literature has informed our hypothesis \chelsea{should I talk about specific literature and hypothesis here? Or in RW?} that encountering AI misrepresentation would make students change their perceptions of the AI significantly in the negative way. 

% To examine this question, we calculated the baseline perception measurement for each participant by taking the average score of their perception measurements after seeing the two samples. We then calculated the perception changes for each individual participant by taking the difference between their individual final perception measurement and the baseline perception measurement. This delta value represents their perception changes before and after encountering AI (mis)representation.

% \subsection{Study 1 Finding: Preliminary Analysis on the Effect of AI Misrepresentation on Students' Perception of SAMI}
% To understand whether encountering AI misrepresentation can significantly change students' perception of the AI, we ran Mann-Whitney U test on the perception change value between the two conditions. Given our small sample size of n=20 in study 1, we chose the nonparametric test Mann-Whitney U test to conduct this analysis without assuming normality in our data. Table~\ref{tab:mann-whitney} summarizes the statistics of each perception differences between the two conditions. 

% \begin{table}[]
%     \sffamily
%     \centering
%     \caption{Summary of significance of perception changes between the two conditions. We report Mann-Whitney $U$ test statistics, $p$-values(* $p$\textless0.05, ** $p$\textless0.01, *** $p$\textless0.001), and effect size $r$. Effect size was calculated using the effect size formula for nonparametric test: \(r = \frac{Z}{\sqrt{N}}\)~\cite{fritz2012effect} ,where $N$ is the total sample size.}
%     \begin{tabular}{llll}
%          \textbf{Measure}   &   \textbf{$u$}    &   \textbf{$p$}     &   \textbf{$r$} \\ \midrule
%          Perceived Risk     &   20.5   &   0.028*  &   0.491 \\
%          Benevolence         &   89.5  &  0.003** &   0.66 \\
%          Competence         &   92    &     0.002** &   0.703  \\
%          Trust (Overall)    &   96    &     0.001** &   0.771 \\
%          Anthropomorphism   &   72      &   0.104   &  0.364 \\
%          Intelligence       &   99   &      0.0002***   &   0.821 \\
%          Likeability        &   90    &     0.003**     &   0.668 \\ \bottomrule
%     \end{tabular}
%     \label{tab:mann-whitney}
% \end{table}


\subsection{Study 1 Findings: Interpreting and Reacting to AI after Encountering AI (Mis)representation}
% In this section, we present our findings from Study 1 to explore students' perception and reaction to SAMI after encountering AI (mis)representation. 

We first confirmed that our manipulation of SAMI inference accuracy was largely effective. We compared students' baseline accuracy rating of SAMI's inferences after seeing the samples and their experiment accuracy rating of SAMI's inferences after seeing their own inferences. We found that in the accurate condition, the accuracy rating largely increased from baseline rating to experiment rating, with a median increase of 1 out of 5; in the inaccurate group, the accuracy rating largely decreased from the baseline rating to the experiment rating, with a median decrease of 0.5 out of 5. However, it is worth mentioning that some participants' accuracy ratings did not change between baseline and experiment (n=1 in the accurate condition, n=3 in the inaccurate condition).

Next, we present our findings from Study 1 to understand students' reactions and perceptions of SAMI after encountering AI (mis)representations. We first describe three rationales that participants adopted through knowledge acquired from SAMI (mis)representations to interpret how SAMI worked: SAMI works like a machine, a human, and/or magic. We then describe participants' reactions of over-trusting, rationalizing, and forgiving of SAMI misrepresentations, highlighting that these reactions were highly connected to the rationales that we pinpointed. 
% Finally, we show that various dimensions of participants' perceptions of SAMI all significantly decreased after encountering SAMI misrepresentations. 

% These three rationales governed their reactions to SAMI's (mis)representations of them--- we found that participants had a tendency to over-trust SAMI's misrepresentations of them, believing that SAMI works like magic; but also tended to rationalize and justify SAMI's misrepresentations, believing that ``SAMI is just a machine.'' Finally, we describe participants' conflicting attitudes towards seeing and sharing SAMI's inferences about them, worrying about SAMI spreading negative images about them in human communities based on the belief that SAMI's inferences could have the same effect as human inferences; yet, sometimes simultaneously, showed indifference about the consequence of sharing SAMI's inferences, believing ``it's just an AI.''

% People hold different rationales of how SAMI works: machine, human, magic. These rationales can co-exist at the same time. When AI exhibit unexpected behaviors, this cause a change or a shift in the dominant rationale that people resorted to at the time. This shift depends on their AI literacy and how much they could make sense of the AI output, and how unexpected AI outputs are. These rationales could explain to some extent of people's reactions to AI behaviors. 
% Over-trusting: SAMI works like magic
% Rationalization: SAMI works like machine
% Forgiving: SAMI works like human


\subsubsection{Interpreting SAMI: Machine? Human? Or Magic?}
Based on our interviews with the participants, we found that participants acquired new knowledge from SAMI (mis)representations. Such newly acquired knowledge prompted participants to adopt different rationales to interpret how SAMI worked: SAMI works like a machine, human, and/or magic. These rationales could co-exist at any given time, yet are bounded by participants' existing AI knowledge, tech proficiency, and how much they could make sense of SAMI's specific inferences. 

\textbf{``SAMI works like a machine.''} The first rationale participants held was that SAMI followed the typical ``input-processing-output'' machine working mechanism. About a quarter of the participants in our study, half of whom self-rated as ``Expert'' in terms of their tech proficiency, could clearly explain how SAMI came up with specific inferences by specifying their perceived SAMI knowledge base, training, input processing, and inference generation process. 
% For example, when asked about how he thought SAMI generated these inferences in the sample, P37 described SAMI's training process,~\textit{``Probably SAMI was trained on a bunch of responses like this. Then maybe someone else labeled how the person actually is, then SAMI was able to learn the different traits out of the writing.''} 
P23 described her speculation of how SAMI processed the self-introduction input to generate personality inferences:~\textit{``From a personality standpoint, I'd imagine that it's sectioning out facts and being like, people who do this are commonly [like] that. And then kind of filtering through several things that point to this person being generally trusting. So in this sample, this person want to travel, want to visit the seven wonders of the world, maybe all of that means they are generally trusting.''}

\textbf{``SAMI works like a human.''} We also observed the ``SAMI works like a human'' rationale surfacing among some participants, all of whom self-reported their tech proficiency as ``Intermediate.'' These participants believed that SAMI drew personality inferences in similar ways as how humans would do it. For instance, P14 described how SAMI worked like humans when coming up with inferences:~\textit{``I think they are probably like us, where [certain things] kind of tick SAMI off. Like maybe people who love to travel can be a little bit more easily distracted, or maybe a little bit more careless, just because they have to be more go with the flow. ''} 
% When asked about SAMI's inference accuracy, most participants compared SAMI's inferences with the kind of inferences they themselves could draw from the intro and said SAMI's inferences were accurate when it's similar to what they could infer, and vice versa. Some participants also described SAMI's inference-making process by attributing personality traits associations that were not common patterns, but unique to their lived human experience. For example, P14 speculated how SAMI came up with the inference of ``you have a forgiving nature'' about her:
% \begin{quote}
%     \textit{``Uhm, I don't necessarily know where they got that one from, but I said I like to facilitate important discussion, and lead others. I feel like, a quality that most people have when they lead a group is, they have to be understanding and somewhat forgiving. Or else, you're never gonna get anything done, because you're just gonna get frustrated with people. So I guess maybe that's where that conclusion came from. (P14)''} 
% \end{quote}
When P16 also described her rationale of how SAMI came up with inferences like humans would, she elaborated:~\textit{``So it's funny, because I know [humans and AI] are not the same at all. But I think like, who's making the AI technology--- people! So maybe the people try to make it think like how we think, even though it's not one and the same. Maybe whoever coded it tried to make it like human perception. ''}

~\textbf{``SAMI works like magic.''} When participants couldn't make sense of SAMI's unexpected inferences from the given self-introduction paragraph, they would sometimes resort to the belief that SAMI was a powerful, knowledgeable, ``big black box of magic.'' This rationale was mentioned by participants with varying levels of tech proficiency. Participants who adopted the magic rationale often could not clearly articulate how SAMI came up with the specific inferences, but instead loaded their answers with vague terms to emphasize the massive amount of training data SAMI might have access to or the ``magical power'' of AI to identify patterns that humans cannot see. For example, P36 who self-rated as an ``Expert'' in tech proficiency explained why he thought some of SAMI's inaccurate inferences about him were true:~\textit{``I was under the impression that it somehow drew inferences... since I didn't see where it got that from, I thought it was drawing inferences from different sources of information, and somehow using a pattern, like using a neural net or something. So I was like `Ok, sure maybe I can see that.' But if a person just told me that and I just don't see where they got it from, then I'd just think the person is being inaccurate. (P36)''}

% Compared to the machine rationale, participants following the magic rationale weren't able to articulate clearly SAMI's processing mechanism but instead emphasized heavily on the massive amount of training data SAMI might have access to. Participants who self-rated as ``Expert'' in tech proficiency would load their answers with vague machine learning terms to obscure their lack of understanding into SAMI's processing mechanism, whereas participants who reported as not familiar with AI held a general belief that AI could read and process a huge amount of data that humans cannot, could identify patterns that humans cannot see, and hence acting somewhat like magic. 
% For example, P36 explained why he thought some of SAMI's inaccurate inferences about him were true:
% \begin{quote}
%     \textit{``I was under the impression that it somehow drew inferences... since I didn't see where it got that from, I thought it was drawing inferences from different sources of information, and somehow using a pattern, like using a neural net or something. So I was like `Ok, sure maybe I can see that.' But if a person just told me that and I just don't see where they got it from, then I'd just think the person is being inaccurate. (P36)''}
% \end{quote}
% Many participants who reported as not familiar with AI held a general belief that AI could read and process a huge amount of data that humans cannot, could identify patterns that humans cannot see, and hence acting somewhat like magic. For example, P26 described his understanding of AI towards the end of his session:~\textit{``I'm not an AI guy. It's just a big black box of magic. I really don't fully understand how AI works. It's just a big abstraction of like, there is this data set, and it finds patterns, and then it uses those patterns. But what's happening under the hood, it's a black box industry.''}  When asked about why they believed some of the inferences could be true, P21 said,~\textit{``It was always like, you know, this could be true. These could be totally true facts that my human brain cannot comprehend, but the AI can. I almost felt... I didn't feel qualified to evaluate SAMI.''}

% P28 also echoed this thought when asked about why she almost trusted some of SAMI's inferences:~\textit{``I know that artificial intelligence is able to analyze large amounts of data from its past, and like, learn about things. So I was like, maybe they just know so well, maybe SAMI just know so well that this student have these qualities.''}


\subsubsection{Reacting to AI Misrepresentation: Over-trusting, Rationalizing, and Forgiving}
% \subsubsection{Trusting and Rationalizing AI Misrepresentations}
% When encountering AI misrepresentations, participants either trusted SAMI's intentionally inaccurate inferences about themselves due to overtrust in AI, or rationalize SAMI's inaccurate inferences citing that these hyper-personalized inferences are difficult for AI to draw. 

After being shown SAMI's inaccurate personality inferences about them, participants displayed a range of reactions: some participants believed there was some truth to  SAMI's misrepresentation; some participants rationalized it and blamed themselves instead; some participants were forgiving of SAMI's mistakes. These reactions to SAMI misrepresentations seemed to be connected to the rationale participants adopted after acquiring new knowledge from SAMI misrepresentations about them. 

\textbf{Over-trusting SAMI Misrepresentations.} 
% To our surprise, we found that some participants in the inaccurate condition believed some of SAMI's inaccurate inferences about them. Given that we intentionally made every SAMI inference to be intentionally inaccurate and the complete opposite of participants' personality ground truth, we expected most participants in the inaccurate condition to rate SAMI's inferences about them as ``1-Not accurate at all.'' However, only two out of 10 participants did so. Six out of 10 participants felt there were a little bit of truth to SAMI's inferences about them by rating SAMI's accuracy as a two out of five, and two participants rated SMAI's inference accuracy about them as ``3-Somewhat accurate.''
% We further unpacked this phenomenon through our qualitative analysis of the interviews and identified several potential reasons why participants tended to believe SAMI's inaccurate personality inferences about them.
To our surprise, we found that most participants in the inaccurate condition often found some truth to SAMI's inaccurate inferences about them. Given that we made every SAMI inference to be intentionally inaccurate and the complete opposite of participants' personality ground truth, we expected most participants in the inaccurate condition to rate SAMI's inferences about them as ``1-Not accurate at all.'' However, only two out of 10 participants did so--- rest of the participants displayed varying levels of trust in SAMI's inaccurate inferences about them, ranging from two to ``3-Somewhat accurate''

These participants often fell into the trap of the Barnum effect~\cite{dickson1985barnum}, a cognitive bias phenomenon that people tend to believe in personality descriptions of them as customized to them, when in fact, these descriptions are often vague and general. When presented with SAMI's inferences about them, participants had a tendency to look for evidence in their daily lives to support SAMI's claims. 
% For example, P24 explained why she saw some truth in SAMI's intentionally inaccurate inference about her``You are disorganized'', which she rated as ``2-Disagree'' on her personality test in the preliminary survey:~\textit{``It just really depends on like, scenarios, like what kind scenarios I'm in? Like, I can be disorganized sometimes. But like in terms of schoolwork, I will say I'm pretty organized. So if you asked me, during teamwork, am I organized? During schoolwork, am I organized? Then I'll probably say yes.''}
In addition, believing in the authority of the evaluator could make the Barnum effect stronger~\cite{dickson1985barnum}. We found that participants in the inaccurate condition displayed a tendency to perceive SAMI as an authority figure that was ``smarter and more powerful'' than them, with opaque working mechanism. 

This echoed with the ``SAMI works like magic'' rationale that they don't know how AI works, but it just should work. This rationale was even present when participants were confident that SAMI's inferences were very inaccurate. For example, P28 rated SAMI's inferences as very inaccurate, yet still took a huge sigh of relief when we told her SAMI's inferences about here were fabricated to be inaccurate:~\textit{``I feel better now because I was worried. I was worried that, because I don't see myself from the outside so I was worried that SAMI was real and kind of accurate, and this is how people see me. ''} She further explained about her reasoning:
% \begin{quote}
\textit{``I guess partly because it's an AI. Because AI is a lot smarter than me. And I don't consider myself to be a computer science expert. AI is so unfamiliar to me that I don't really know what is the line between true and false. I don't know when to trust it or not to. I think with SAMI, I was erring on the side of being not trusting but then deep inside, I was like, `this is an AI, it's really smart, it should be able to know.' I think that's why I felt like I could trust it. After I saw the two samples and then when it came to mine, I started to feel like something was wrong. Uhm, but then deep down I was like, `ok, well, maybe it is right.'''}
% \end{quote}

\textbf{Rationalizing SAMI Misrepresentations.} Besides participants' tendency to over-trust AI misrepresentations, we also found that participants had a tendency to rationalize AI mistakes, or ``find excuses'' for SAMI's inaccurate inferences. When participants noticed that SAMI's inferences might not be accurate for either the students in the sample or themselves, some participants would ``justify'' SAMI's inaccuracies, citing it could be a result of the nature and quality of the self-introductions. This echoed with the ``SAMI works like a machine'' rationale that participants believed ``unqualified'' input would hurt the machine's output. For instance, when P29 spotted SAMI's inaccurate inferences in one of the samples, she said,~\textit{``I feel like the person was fairly broad in what they wrote. And so that also could have influenced SAMI's response. Like it didn't necessarily go too in-depth, [...] It also went from learning languages, study abroad, and then the career of helping people. That could have thrown SAMI off a little bit as well, seeing as it like, it bounced around a little bit more. ''} P36 also said that SAMI might have made inaccurate inferences about him due to him not mentioning certain things in his self-introduction:~\textit{```You can be somewhat careless.' I would say that is like very inaccurate. I'm a very meticulous person. But I guess I never really touched on that anywhere in my response...''}

\textbf{Forgiving SAMI Misrepresentations.} Many participants were forgiving of SAMI's misrepresentations of either themselves or students in the samples. This echoed the ``SAMI works like a human'' rationale in that this reaction is analogous to how they would react to human mistakes. After encountering SAMI misrepresentations, participants attributed good intentions and efforts to SAMI. Following this line of reasoning, participants believed that just like human mistakes, SAMI's mistakes could be forgiven considering its good intentions and efforts. This reaction was presented in more than half of the participants in the inaccurate condition. After reviewing SAMI's misrepresentations of themselves, they believed that SAMI was ``trying'' and well-intentioned, but just not as capable as they expected. Some participants in the accurate condition, noticing that SAMI did not make perfect inferences in the samples, were still hopeful about SAMI despite its mistakes. P29 said,~\textit{``[I'm thinking of] a little kid where they want to help out and be like `oh my gosh, look what I did' and presented it to you and be like `Look, I'm trying to be helpful.' But it's not always the most helpful or accurate in this situation. I was thinking that [SAMI] is trying to help, it is generating those responses, but at the same time, it just might not be the most accurate.''} 

% \subsubsection{Sharing AI Misrepresentations: Should I be Concerned?} During the interviews, we asked participants about their potential concerns or perceived risks of sharing SAMI's inferences with others or when the inferences were used for team matching. We found that participants in our study exhibited a somewhat ``conflicted feeling'' about sharing AI (mis)representations. 

% On the one hand, some participants expressed concerns about negative team-matching results based on SAMI's inferences about them. More than half of the participants worried that SAMI might spread inaccurate, or even negative, impressions of them, which would not only hurt their team-matching results but also be detrimental to their reputations among their classmates. For example, P37 said,~\textit{``Um, I wouldn't want my teammates to see some labeled traits about me and immediately assume that to be true. I'd rather they judge me throughout the project.''} P17 also echoed this concern when asked about SAMI performing team matching based on the inferences generated about her:~\textit{``If it was unedited, then I don't think I would feel very good about it. Mainly because it makes me sound, like very rude. Like I'm rude to others, and I start arguments with other people. I think if it was unedited, then I wouldn't want to use it to be put into the team. (P17)''}

% Some participants were worried that SAMI's inferences might seem offensive to some people, or even hurt their feelings. P14 described her initial reaction when seeing SAMI's inferences in the samples:~\textit{``At first, I was a little offended for this person. Because I was like `Oh, this AI software is saying you are careless and easily distracted.'''} P22 also said,~\textit{``A lot of them are just kind of stated very bluntly. Like, for example, `you're sometimes rude to others.' I think some people might be hurt by that.''}

% About half of the participants also expressed their concerns that people might change their self-perceptions based on SAMI's inferences about them, which could be inaccurate. For instance, P21 said:
% \begin{quote}
%     \textit{``Like those last two sentences in the first sample, `you can be somewhat careless,' `you are easily distracted.' Maybe they didn't think of themselves as careless or distracted. They are like, `oh if this AI model is saying that I am, then maybe I am.' So it might get people a little confused and maybe frustrated or sad, and they feel like they don't know themselves as well as they do, or as well as they thought they do. (P21)''}
% \end{quote}


% % P37 said he didn't like the idea of machines putting labels on people and then showed the labels to people. When asked to elaborate, P37 said,~\textit{``Yeah [I don't want to see the label]. I could illustrate um, I forgot what it's called, but whenre you see that you are labeled that way, you might start to act that way more and maybe it takes away some of your free decisions. ''}

% On the other hand, some participants, even some of the participants who voiced concerns about sharing AI misrepresentations early on, dismissed some of the concerns and risks mentioned because ``it's just an AI.'' P23 described her somewhat conflicted reactions when reading SAMI's inferences about her:~\textit{``Part of me says, `ouch, kind of rude.' But the other part of me is like, it's an AI, it's not meant to take into account of how I would feel when reading this. So, overall, I wasn't hurt by the paragraph. Sometimes I read it and it's like, damn. But, no, I think it's all right. I wasn't like super-duper offended. ''} P21, who pointed out the potential risks of people changing their self-perceptions based on SAMI's inferences earlier, later dismissed most of that concern after reading their own inferences:
% \begin{quote}
%     \textit{``I think at that point, I was just feeling like,  if you read something, and it doesn't feel accurate, and it's from an AI model, you can be like, `Okay, it's an AI model.' I am myself, I have spent however many years of myself. I guess that people would be able to discern for themselves, and not take [SAMI's inferences] on them as a way to go back and forth between those two. (P21)''}
% \end{quote}

% P33, who also voiced concerns about SAMI's inaccurate inferences spreading negative impressions of people when not accurate, also added later that he was not too concerned about it because he trusted that students would have the time and opportunity to clear up any misjudgments caused by SAMI: 

% \begin{quote}
%     \textit{``Um, I don't think it's super serious because if someone was to be put in a group with someone, there's always going to be a discourse at the beginning because they're still getting to know each other. And you don't really know those people in your group until after you have more time to talk to like clear things up. So I don't think [SAMI's inferences] would completely eliminate him from being on a team. (P33)''}
% \end{quote}

% We noticed the concerns largely treated AI misrepresentations as having the same effectiveness as human-generated negative impressions of them, which could be based on the human rationale; the lack of concerns often dismissed AI misrepresentations as generated by a machine and therefore unreliable to capture human traits, which could be based on the machine rationale. Participants raising concerns but then dismissing the concerns could be indicative of their ``rationale switch'', where participants quickly switched from the human rationale to the machine rationale when they realized that it's just an AI, and AI's output should not be treated like human-generated information. 

% % Despite the somewhat conflicted feelings about the potential risks and concerns about sharing AI misrepresentations, majority of the participants said they would like to check or edit SAMI's inferences before SAMI shares it out with others. Some participants also expressed their desire to engage with SAMI in a back-and-forth conversation to improve the accuracy of SAMI's understanding of them.


% % When asked about whether he would be willing to share SAMI's inferences with others such as professors and her classmates, P35 said,~\textit{``I feel like I want to be able to see the inferences first and make sure it’s accurate enough. I guess, if I just blindly tell the agent do whatever you want, I would definitely not be in any team if SAMI shares this. Yeah I don’t think I’m very comfortable with the AI agent taking control without a human in the loop.  (P35)''} 

% % Other participants also expressed their desire to engage with SAMI in a back-and-forth conversation to improve the accuracy of SAMI's understanding of them. P17 said:
% % \begin{quote}
% %     \textit{``As a person, I can get opinion about somebody just reading a little introduction. For an AI it would probably be a little harder. So you would need the back and forth just so like, at the end of the day, if you're using SAMI for a group project, you want to be paired with people that you would actually get along with and work well with. So I wouldn't mind like talking back and forth just so he can get the description as accurate as possible. (P17)''}
% % \end{quote}



==> source/5study2.tex <==
\section{Study 2: Examining the Changes in Students' Perception of AI after Encountering AI Misrepresentations}
To explore the changes in students' perceptions of AI (RQ2 and RQ3) after encountering AI misrepresentations, we conducted a survey experiment on Prolific and solicited a larger sample to quantify the changes in student perceptions as well as contributing factors to the changes. Similar to Study 1, we first deployed a preliminary survey to collect information for fabricating students' personality inferences. Then after a week, we followed up with an experiment survey to show participants SAMI's inferences and measured their perception changes of SAMI. Based on our observations from Study 1, we added a general AI literacy measurement in the preliminary survey to examine AI literacy as a potential factor contributing to the changes in students' perceptions of AI after encountering AI misrepresentation. 
% Specifically, study 2 aimed at answering two specific research questions:

% \begin{table}[h]
% % \sffamily
% \centering
% % \footnotesize
% \vspace{-0.5em}
% \begin{tabular}{@{}l@{}p{0.92\columnwidth}@{}}
%     \textbf{RQ 3.1: } & What is the effect of AI misrepresentation on students' trust and social perceptions of the AI?  \\
%     \textbf{RQ 3.2: } & How does students' levels of AI literacy moderate the effect of changes in students' perception of AI after encountering AI misrepresentation? \\
%     % \bottomrule
% \end{tabular}
% \vspace{-0.9em}
% \end{table}


\subsection{Study 2 Study Design}
% Study 2 consisted of two surveys: the preliminary survey to collect students' basic background information, their AI literacy, and their personality ground truth; the experiment survey, distributed at least a week after the preliminary survey, to show students SAMI's fabricated inferences about them and collect their perceptions of SAMI. 

We deployed the preliminary survey (see Supplementary Materials~\ref{supp:s2_prelim_survey}) on Prolific and recruited current students above age 18 of all study levels in the United States. Participants were told that the goal of this study was to understand students' perception of a team-matching AI agent. In the preliminary survey, participants provided their self-introduction paragraph, responses to the personality test and an AI literacy questionnaire, as well as their demographic, background, and team project experience information. Participants who completed the preliminary survey were compensated with \$3 USD. The median completion time was 11 min and 41 seconds. 

250 Prolific participants filled out our preliminary survey on Qualtrics. We removed seven participants whose self-introductions were suspected to be generated by generative AI tools such as ChatGPT. Given our emphasis on AI misrepresentation in Study 2, we assigned about 70\% of the participants to the inaccurate condition and about 30\% of the participants to the accurate condition. We then wrote a Python script to fabricate SAMI's inferences for the 243 remaining participants following the same fabrication procedure and guidelines in Study 1. By following the 60\% positive and 40\% negative inference ratio rule, we removed 21 participants since their fabricated inferences were either too positive or too negative based on their personality ground truth. This resulted in 222 participants remaining (n=157 in inaccurate condition, n=65 in accurate condition), all of whom were invited to participate in the experiment survey. 

The experiment survey (see Supplementary Materials~\ref{supp:s2_exp_survey}) followed the Study 1 procedure by showing the same two samples and prompted participants to answer their perceived accuracy of SAMI inferences, as well as filling out measurements of their trust and social perceptions of SAMI. Participants then retrieved SAMI's inferences about them by entering their Prolific ID on a website that we created (see Appendix~\ref{appendix:s2website}), and then filled out the same perception measurements. Finally, a debriefing form informed participants about the real purpose of the study and how SAMI's inferences were fabricated. Participants were compensated with \$3 USD for completing the experiment survey, and an extra \$4 USD bonus for completing both surveys. We received 211 responses (n=151 for inaccurate condition, n=61 for accurate condition) for the experiment survey. The median completion time was 12 min and 43 seconds. A description of the perception measures and general AI literacy measures used in Study 2 can be found in Appendix~\ref{appendix:s2measures}.

After we concluded the data collection, we removed 13 participants' data due to extremely fast completion time (less than six minutes) and obvious contradictions in their responses. We ended up with 198 participants' data for the experiment survey, with 57 participants in the accurate condition and 141 participants in the inaccurate condition. 

% \subsection{Study 2 Measures}
% In this section, we describe the three scales that we used in the preliminary survey and the experiment survey: the General AI Literacy Scale measures AI literacy as our moderator, the Human-Computer Trust scale measures students' trust in SAMI as one of the four outcomes, and the Godspeed scale for human-robot interaction measures perceived intelligence, anthropomorphism, and likeability of SAMI as the remaining three outcomes.

% \textbf{General AI Literacy Scale: } This 13-item scale was developed and validated by~\citeauthor{pinski2023ai} to measure general AI literacy, which they interpreted as ``humans' socio-technical competences regarding AI''~\cite{pinski2023ai}. This scale consists of five dimensions: AI technology knowledge, human actions in AI knowledge, AI steps knowledge, AI usage experience, and AI design experience. The responses were recorded on a five point Likert scale. Our correlation test suggested that the five dimensions were highly inter-correlated in our sample, with correlation ranging from 0.31 to 0.73. To avoid inflating our regression model, we decided to use an overall literacy score that is the sum of the score for each dimension. 

%%%%% explain the two significant moderator in post-hoc
% This general AI literacy scale measures five dimensions of general AI literacy:~\textit{AI technology knowledge}, which measures participants' knowledge regarding what makes AI distinct from other technology and the role of AI in human-AI interaction;~\textit{Human actions in AI knowledge}, which measures participants' knowledge of the role of human actors in human-AI interaction; ~\textit{AI steps knowledge}, which measures participants' knowledge about AI's input, processing, and output and each step's impact on humans;~\textit{AI usage experience}, which measures participants' use experience with AI;~\textit{``AI design experience''}, which measures participants' experience in designing and developing AI models and/or AI-driven products. 

% An overall AI literacy score was calculated by taking the sum of the score for each AI literacy dimension given that these dimensions are highly correlated with each other. We found these dimensions are highly inter-correlated, ranging from XX to XX. For the sake of simplicity in our model, we decided to use an overall literacy score that captures all these dimensions by taking the sum of them. \chelsea{@vedant I forgot why we decided to take the sum of all the AI lit dimensions... Was it because they were all highly correlated? And if so, how should I report the correlation here?}

% \textbf{Human-Computer Trust Scale:} We measured students' trust in SAMI by using the ``Human-Computer Trust Scale'' developed and validated by~\citeauthor{gulati2019design}. This scale consists of 12 statements that can be customized to the specific AI technology being studied, and responses were recorded on a five-point Likert scale. This scale measures four dimensions of trust: perceived risk, benevolence, competence, and overall trust. Given that the scores for each of the dimensions were highly inter-correlated, with correlation magnitude ranging from 0.45 to 0.75, we took the score for overall trust to represent participants' trust in SAMI in our analysis. 

% \textbf{Godspeed Scale for Human-Robot Interaction:} We measured students' social perceptions of SAMI by using the Godspeed scale developed and empirically validated by~\citeauthor{bartneck2009measurement}. This scale has been commonly used to measure users' social perception of AI agents in prior literature ~\cite{wang2021towards,mirnig2017err,honig2018understanding,salem2015would}. This scale is a semantic differential scale that asks participants to indicate their position on a scale between two bipolar words (e.g., Fake 1 2 3 4 5 Natural). We adapted the scale and took the three dimension measurements that were applicable to SAMI:~\textit{Anthropomorphism, Perceived Intelligence, and Likeability.}~\textit{Anthropomorphism} measures participants' level of attribution of human forms or human characteristics to the agent;~\textit{Perceived Intelligence} measures participants' perception of how smart or intelligent the agent is;~\textit{Likeability} measures participants' level of positive impression of the agent. 

\subsection{Study 2 Participant Summary}
% From Vedant: For Study 2: You can move the equations inline. Also when you're giving a participant summary, you do not have to describe all proportions inline itself. You can simply mention the highest percentages (E.g., 70% were UG). Similarly for scores you can mention "The mean extraversion was 2.1±0.1". Generally the more detailed numbers are in a table.

Our final participant pool (n=198) has an average age of 31.3±11.12, ranging between 18-74 years old. 42.9\% were women, 53.5\% were men. Most students were at the undergraduate level (n=146, 73.7\%). 46.5\% students in non-STEM major, 52\% in STEM major. Participants were relatively familiar with AI, with an average of 14.3±4.50 out of 25 on overall AI literacy.
% In our final participant pool (n=198), the average age was 31.3 (median=28, SD=11.12, range=18-74). Among the participants, there were 42.9\% women (n=85), 53.5\% men (n=106), 0.03\% non-binary (n=5), 0.01\% prefer not to say (n=1), and 0.01\% prefer to self-describe (n=1, self-described as ``agender''). There were 73.7\% currently studying at the undergraduate level (n=146), 17.2\% at the master level (n=34), 0.02\% at the doctorate level (n=3), and 0.03\% described as other level (E.g., Gen.Ed., associate degree). There were 46.5\% studying non-STEM major (n=92), 52\% studying STEM major (n=103), with 0.02\% not specified (n=3). Participants were relatively familiar with AI, with an average of 14.3 out of 25 on overall AI literacy (median=14.41, SD=4.50, range=5--25).
Participants were generally experienced in team projects at school, having participated in an average of 12 team projects (median=5, SD=25.8, range=0--300). Participants held a relatively positive attitude about their team project experience, reflected in an average rating of 3.7 ± 0.88 out of a five-point Likert scale. 
% Eight participants didn't report given they had not been involved in any team projects.
We provided more details about the participants' demographic and personality in Appendix~\ref{appendix:s2_participant}.
% Given that personality could affect students' perception of AI after personality misrepresentations, we also summarized and provided an overview of the participants' personality along the five Big-Five dimensions in the supplementary material. 


% provide an overview of the participants' personality (on a scale from 1 to 5): the average of participants' Extroversion is 2.93 (median=2.88, SD=0.86, range=1--5), the average of participants' Agreeableness is 3.86 (median=3.88, SD=0.66, range=2.22--5), the average of participants' Conscientiousness is 3.79 (median=3.78, SD=0.73, range=1.67--5), the average of participants' Neuroticism is 2.83 (median=2.88, SD=0.99, range=1--5), and the average of participants' Openness is 3.76 (median=3.8, SD=0.65, range=1.6--5)

\subsection{Study 2 Data Analysis}
We first calculated the changes in students' perceptions of SAMI (overall trust, anthropomorphism, perceived intelligence, likeability) by taking the difference between students' baseline perceptions ($B_p$) and experiment perceptions ($E_p$): $\Delta= E_p - B_p$. We then coded condition as 0 (accurate condition) and 1 (inaccurate condition) during analysis.

To understand the effect of AI misrepresentation on students' perception changes of SAMI (RQ2), we performed four sets of linear regressions with the $\Delta$ of each perception construct as the outcome and the participants' condition as the independent variable. We controlled for age, gender, study level, major (STEM or non-STEM), number of projects, project experience rating, and five personality dimensions. Equation~\ref{eq1} describes our linear regression models, where$\Delta~\mathcal{P}$ refers to changes in overall trust, anthropomorphism, intelligence, and likeability. 
\vspace{-0.1in}
\begin{multline}
\label{eq1}
\small
    \Delta\mathcal{P} \sim Condition + Age + Gender + Study Level + Major + Project Count + Project Experience \\+ Extroversion + Neuroticism + Agreeableness + Openness + Conscientiousness
\end{multline}
\vspace{-0.2in}

To understand the moderating effect of AI literacy (RQ3), we again performed four sets of linear regression models, but this time incorporating AI literacy. Specifically, we performed two versions of linear regression for each model: one that included AI literacy (Equation~\ref{eq2}), and another included AI literacy plus an interaction effect between AI literacy and condition (Equation~\ref{eq3}). We included the only significant covariate from prior models--- the Openness personality dimension. The outcome $\Delta \mathcal{P}$ is the changes in overall trust, anthropomorphism, intelligence, and likeability. 
% \vspace{-0.03in}
\begin{equation}
    \label{eq2}
    \small
    \Delta\mathcal{P} \sim Condition + AI Literacy + Openness
\end{equation}
\vspace{-0.2in}

\vspace{-0.2in}
\begin{equation}
\label{eq3}
\small
    \Delta\mathcal{P} \sim Condition + AI Literacy + Condition * AI Literacy + Openness
\end{equation}
\vspace{-0.15in} 


\subsection{Study 2 Findings}
Our results show that encountering AI misrepresentations had a significant effect on changes in students' overall trust, perceived intelligence, anthropomorphism, and likeability of SAMI. We also found that AI literacy could moderate the effect of AI misrepresentations on changes in students' overall trust in SAMI, but not their social perceptions of SAMI. 

% \subsubsection{Students' Changes in Perceptions of SAMI}
% We report the descriptive statistics of students' changes in perceptions in Table~\ref{tab:perception_changes}. We saw a general trend of students in the accurate condition increasing their perceptions of overall trust, perceived intelligence, anthropomorphism, and likeablity of SAMI after being shown an accurate personality portrayal of themselves by SAMI. We also observed a general trend of students in the inaccurate condition decreasing their perceptions of overall trust, perceived intelligence, anthropomorphism, and likeability of SAMI after being shown an inaccurate personality portrayal of themselves. This showed us that our manipulation to the accuracy of SAMI's inferences worked as we expected. 

% % In baseline perceptions measured after students were shown the samples, in terms of overall trust in SAMI, students in the accurate condition had an average rating of 2.42 out of 5 (median=2.33, SD=1.04, range=1--4.33); students in the inaccurate condition had an average rating of 2.14 out of 5 (median=2, SD=1.02, range=1--4.67). In terms of perceived intelligence of SAMI, students in the accurate condition had an average rating of 3.18 (median=3.4, SD=1.09, range=1--5); students in the inaccurate condition had an average rating of 2.99 (median=3, SD=0.95, range=1--5). In terms of perceived anthropomorphism of SAMI, students in the accurate condition had an average rating of 2.41 (median=2.2, SD=1, range=1--5); students in the inaccurate condition had an average rating of 2.25 (median=2.2, SD=0.83, range=1--4.8). In terms of likeabilty of SAMI, students in the accurate condition had an average rating of 3.24 (median=3.2, SD=1.01, range=1--5); students in the inaccurate condition had an average raing of 3.04 (median=3, SD=0.79, range=1--4.8).

% % In experiment perceptions measured after students were shown intentionally inaccurate or accurate SAMI inferences about them, in terms of overall trust in SAMI, students in the accurate condition had an average rating of 3.01 (median=3.33, SD=1.08, range=1--4.67); students in the inaccurate condition had an average rating of 1.61 (median=1, SD=0.91, range=1--4.67). In terms of perceived intelligence of SAMI, students in the accurate condition had an average rating of 3.54 (median=3.8, SD=1.07, range=1--5); students in the inaccurate condition had an average rating of 2.43 (median=2.4, SD=0.97, range=1--5). In terms of perceived anthropomorphism of SAMI, students in the accurate condition had an average rating of 2.65 (median=2.4, SD=1.1, range=1--5); students in the inaccurate condition had an average rating of 1.98 (median=1.8, SD=0.85, range=1--4.8). In terms of likeabilty of SAMI, students in the accurate condition had an average rating of 3.47 (median=3.4, SD=1.02, range=1--5); students in the inaccurate condition had an average raing of 2.67 (median=2.8, SD=0.83, range=1--5).

% % We calculated changes in perception after encountering AI (mis)representation by subtracting baseline perceptions from the experiment perceptions. In terms of changes in overall trust in SAMI, students in the accurate condition had an average change of 0.6 (median=0.3, SD=0.75, range=-0.3--3); students in the inaccurate condition had an average change of -0.53 (median=-0.3, SD=0.79, range=-3.67--2). In terms of changes in perceived intelligence in SAMI, students in the accurate condition had an average change of 0.37 (median=0.2, SD=0.69, range=-1--2.4); students in the inaccurate condition had an average change of -0.56 (median=-0.4, SD=0.73, range=-3.2--1). In terms of changes in perceived anthropomorphism in SAMI, students in the accurate condition had an average change of 0.24 (median=0, SD=0.57, range=-1.4--2.2); students in the inaccurate condition had an average change of -0.27 (median=-0.2, SD=0.57, range=-3.2--1.4). In terms of changes in likeability of SAMI, students in the accurate condition had an average change of 0.24 (median=0, SD=0.49, range=-0.4--1.4); students in the inaccurate condition had an average change of -0.38 (median=-0.2, SD=0.725, range=-3.8--1.4).

% \begin{table}[]
%     \centering
%     \sffamily
%     \footnotesize
%     \caption{Descriptive statistics for changes in perceptions, aggregated by condition}
%     \begin{tabular}{lllll}
%            &   \textbf{Mean}    &   \textbf{Median}  &   \textbf{Std} &   \textbf{Range} \\ \toprule
%          \textbf{Accurate Condition}     &   &   &   &   \\
%          Changes in Overall Trust   & 0.6  &   0.3  &   0.75    & (-0.3, 3) \\
%          Changes in Perceived Intelligence &  0.37  &   0.2 &   0.69    & (-1, 2.4) \\
%          Changes in Perceived Anthropomorphism  &   0.24    &   0   &   0.57    &   (-1.4, 2.2) \\
%          Changes in Likeability     &   0.24    &   0   &   0.49    &   (-0.4, 1.4) \\ \midrule
%          \textbf{Inaccurate Condition} &   &   &   &   \\
%          Changes in Overall Trust   & -0.53  &   -0.3  &   0.79    & (-3.67, 2) \\
%          Changes in Perceived Intelligence &  -0.56  &   -0.4 &   0.73    & (-3.2, 1) \\
%          Changes in Perceived Anthropomorphism  &   -0.27    &   -0.2   &   0.57    &   (-3.2, 1.4) \\
%          Changes in Likeability     &   -0.38    &   -0.2   &   0.73    &   (-3.8, 1.4) \\ \bottomrule
%     \end{tabular}
%     \label{tab:perception_changes}
% \end{table}

% \begin{table}[t]
%     \centering
%     \sffamily
%     \footnotesize
%     \caption{Results of our regression models(Equation~\ref{eq1}) show that participants in the inaccurate condition had a significant decline in overall trust, perceived intelligence, anthropomorphism, and likeability. Only significant covariate, the Openness personality dimension, is reported in the table. *** p<0.001 ** p<0.01 * p<0.05 . p<0.1}
%     \setlength{\tabcolsep}{1.1em}
%     \renewcommand{\arraystretch}{1.2}
%     \begin{tabular}{lcccccccccccc}
%         &   \multicolumn{3}{c}{\textbf{Overall Trust}}   &   \multicolumn{3}{c}{\textbf{Intelligence}}    &   \multicolumn{3}{c}{\textbf{Anthropomorphism}}    &   \multicolumn{3}{c}{\textbf{Likeability}} \\ 
%         &   Est.    &   &   S.E &   Est.    &   &   S.E &   Est.    &   &   S.E     &   Est.    &   &   S.E \\ \toprule
%         (Intercept) &   0.84    &   &   0.782   &   0.64   &   &   0.728   &   -0.06   &   &   0.578   &   1.39    & * &   0.664 \\
%         Openness    &   -0.08   &   &   0.100   &   -0.17   & . &  0.093   &    -0.09   &   &   0.074   &   -0.18   & * &   0.085 \\ \midrule
%         Condition (Inaccurate)   &   -1.14   &***&   0.133   &   -0.92    &***&  0.124   &    -0.50   &***&   0.098   &   -0.58   &***&   0.113 \\ 
%         &   \multicolumn{3}{c}{Adj. $R^2$=0.283***} &   \multicolumn{3}{c}{Adj. $R^2$=0.234***}     &   \multicolumn{3}{c}{Adj. $R^2$=0.111***}     &   \multicolumn{3}{c}{Adj. $R^2$=0.139***} \\ 
%         \bottomrule
%     \end{tabular}
%     \label{tab:lm}
% \end{table}


\subsubsection{The Effect of AI Misrepresentation on Students' Perceptions of AI} 
We first looked at students' perception changes before and after encountering AI misrepresentations. We found that students' baseline perceptions in both conditions were similar in terms of overall trust, intelligence, anthropomorphism, and likeability, with a difference in median of less than 0.4 between conditions (details in Appendix~\ref{appendix:s2effectonchanges}). We then plotted out the changes in each perception outcome in density plots (Fig.~\ref{fig:perception_changes_density} in Appendix~\ref{appendix:s2effectonchanges}) and noticed that many participants in the inaccurate condition decreased their perceptions after encountering AI misrepresentations compared to participants in the accurate condition. Therefore, encountering AI misrepresentations seemed to have a negative effect on students' perceptions of SAMI. 

% To understand the effect of AI misrepresentations on students' perceptions of SAMI, we first look at changes in their perceptions after encountering AI misrepresentations. Students' baseline perceptions of SAMI showed that participants in both conditions had similar initial perceptions in terms of overall trust (accurate condition median=2.33, SD = 1.04; inaccurate condition median=2, SD = 1.02), intelligence (accurate condition median=3.4, SD=1.09; inaccurate condition median=3, SD=0.95), anthropomorphism (accurate condition median=2.2, SD=1; inaccurate condition median=2.2, SD=0.83), and likeability(accurate condition median=3.2, SD=1.01; inaccurate condition median=3, SD=0.79). 

% We then looked at the changes in students' perceptions after we introduced SAMI's inferences in the two conditions. We plotted out the changes in each perception outcome in density plots as shown in Fig.~\ref{fig:perception_changes_density}. We noticed that many participants in the inaccurate condition decreased their perceptions of SAMI after encountering AI misrepresentations compared to participants in the accurate condition. Therefore, encountering AI misrepresentations seemed to have a negative effect on changes in students' perceptions of SAMI. 

% \begin{figure}
%     \centering
%         \begin{subfigure}[b]{0.24\textwidth}
%             \centering
%             \includegraphics[width=\textwidth]{source/figures/density_trust.pdf}
%             \caption{}
%             \label{fig:density_trust}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}[b]{0.24\textwidth}
%             \centering
%             \includegraphics[width=\textwidth]{source/figures/density_int.pdf}
%             \caption{}
%             \label{fig:density_int}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}[b]{0.24\textwidth}
%             \centering
%             \includegraphics[width=\textwidth]{source/figures/density_ant.pdf}
%             \caption{}
%             \label{fig:density_anth}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}[b]{0.24\textwidth}
%             \centering
%             \includegraphics[width=\textwidth]{source/figures/density_like.pdf}
%             \caption{}
%             \label{fig:density_like}
%         \end{subfigure}
%     \caption{Density plots visualizing the participant distribution of changes in overall trust, intelligence, anthropomorphism, and likeability in the accurate and inaccurate conditions.}
%     \label{fig:perception_changes_density}
% \end{figure}

% % In baseline perceptions measured after students were shown the samples, in terms of overall trust in SAMI, students in the accurate condition had an average rating of 2.42 out of 5 (median=2.33, SD=1.04, range=1--4.33); students in the inaccurate condition had an average rating of 2.14 out of 5 (median=2, SD=1.02, range=1--4.67). In terms of perceived intelligence of SAMI, students in the accurate condition had an average rating of 3.18 (median=3.4, SD=1.09, range=1--5); students in the inaccurate condition had an average rating of 2.99 (median=3, SD=0.95, range=1--5). In terms of perceived anthropomorphism of SAMI, students in the accurate condition had an average rating of 2.41 (median=2.2, SD=1, range=1--5); students in the inaccurate condition had an average rating of 2.25 (median=2.2, SD=0.83, range=1--4.8). In terms of likeabilty of SAMI, students in the accurate condition had an average rating of 3.24 (median=3.2, SD=1.01, range=1--5); students in the inaccurate condition had an average rating of 3.04 (median=3, SD=0.79, range=1--4.8).

To further examine the effect of encountering AI misrepresentation on students' perceptions of SAMI, we built four linear regression models with changes in each perception as the outcome. Our models show that after controlling for demographics, team project numbers and experiences, as well as the personality dimensions, encountering AI misrepresentation had a significant effect on changes in students' perceptions of SAMI in terms of overall trust, perceived intelligence, anthropomorphism, and likeability (Table~\ref{tab:lm_perceptionchanges} in Appendix~\ref{appendix:s2effectonchanges}). Specifically, participants who encountered AI misrepresentations reported significantly lower overall trust in SAMI (Est.=-1.14, p < 0.001) in comparison to those in the accurate condition. We also found that participants who encountered AI misrepresentations reported significantly lower perceived intelligence (Est.=-0.92, p < 0.001), anthropomorphism (Est.=-0.50, p < 0.001), and likeability (Est.=-0.58, p < 0.001) compared to the participants in the accurate condition. This suggested that after people encountered AI misrepresentation, they were more likely to view the AI as less trustful, less intelligent, less humanlike, and less likable. 

\subsubsection{AI Literacy as a Moderator on the Effect of AI Misrepresentation on Students' Perceptions of AI} We then looked at the possible moderating effect of AI literacy on the effect of AI misrepresentation on the changes in students' perceptions of AI. Our base models that include an effect for AI literacy (Equation~\ref{eq2}) (Models 1a., 2a., 3a., 4a., in Table~\ref{tab:moderation} in Appendix~\ref{appendix:s2_literacy}) show that AI literacy alone does not have a direct relationship with the outcomes; however, our models that include an interaction effect between AI literacy and condition (Equation~\ref{eq3}) (Models 1b., 2b., 3b., 4b., in Table~\ref{tab:moderation} in Appendix~\ref{appendix:s2_literacy}) show that there is a significant interaction between AI literacy and condition on changes in overall trust (Est. = -0.06, p < 0.05). However, this interaction is not significant on changes in intelligence, anthropomorphism, and likeability. Detailed model results can be found in Table~\ref{tab:moderation} in Appendix~\ref{appendix:s2_literacy}. This suggests that students' AI literacy could have an effect on students' overall trust of AI after encountering AI misrepresentations; however, students' AI literacy does not have an effect on students' perceived intelligence, anthropomorphism, likeability of the AI after encountering AI misrepresentation. 

% To examine the moderating effect of AI literacy on students' changes in perceptions after encountering AI misrepresentations, 
Fig.~\ref{fig:literacy_interaction} shows the interaction effect between AI literacy and condition on students' changes in perceptions. 
% in Fig.~\ref{fig:literacy_interaction}. 
In Fig.~\ref{fig:interaction_trust}, students with higher AI literacy were more likely to change their overall trust in SAMI after encountering AI misrepresentations; students with lower AI literacy were less likely to change their overall trust in SAMI after encountering AI misrepresentations. Figures~\ref{fig:interaction_int},~\ref{fig:interaction_anth},~\ref{fig:interaction_like} show the non-significant interaction effect between AI literacy and condition, suggesting that students' levels of AI literacy has no significant effect on their changes in perceptions of intelligence, anthropomorphism, and likeability of the AI after encountering AI misrepresentations.

\begin{figure}
    \centering
        \begin{subfigure}[b]{0.24\textwidth}
            \centering
            \includegraphics[width=\textwidth]{source/figures/trust_lit_interaction.pdf}
            \caption{Overall Trust}
            \label{fig:interaction_trust}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.24\textwidth}
            \centering
            \includegraphics[width=\textwidth]{source/figures/int_lit_interaction.pdf}
            \caption{Intelligence}
            \label{fig:interaction_int}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.24\textwidth}
            \centering
            \includegraphics[width=\textwidth]{source/figures/ant_lit_interaction.pdf}
            \caption{Anthropomorphism}
            \label{fig:interaction_anth}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.24\textwidth}
            \centering
            \includegraphics[width=\textwidth]{source/figures/like_lit_interaction.pdf}
            \caption{Likeability}
            \label{fig:interaction_like}
        \end{subfigure}
    \caption{(a) AI literacy significantly moderated the effect of AI misrepresentations on students' changes in overall trust of SAMI. (b) (c) (d) show that AI literacy does not significantly moderate the effect of AI misrepresentations on students' changes in perceived intelligence, anthropomorphism, and likeability of SAMI.}
    \label{fig:literacy_interaction}
\end{figure}



% \begin{table}[t]
%     \centering
%     \sffamily
%     \footnotesize
%     % \setlength{tabcolsep}{12pt}
%     \caption{Results of our regression models with AI literacy in base models (Equation~\ref{eq2}) and base + interaction models (Equation~\ref{eq3}). Results suggested a significant interaction effect between condition and AI literacy in changes in overall trust after encountering AI misrepresentations. However, significant interaction effect is not found in changes in intelligence, anthropomorphism, and likeability *** p<0.001 ** p<0.01 * p<0.05 . p<0.1}
%     \setlength{\tabcolsep}{1em}
%     \renewcommand{\arraystretch}{1.2}
%     \begin{tabular}{lllllllllllll}
%         &   \multicolumn{6}{c}{\textbf{Overall Trust}}   &   \multicolumn{6}{c}{\textbf{Intelligence}}  \\ 
%         &   \multicolumn{3}{c}{\textbf{1a. Base}}   &    \multicolumn{3}{c}{\textbf{1b. Base + Interaction}}    &   \multicolumn{3}{c}{\textbf{2a. Base}}   &    \multicolumn{3}{c}{\textbf{2b. Base + Interaction}}  \\ 
%         &   Est.    & &     S.E     &   Est.    & &     S.E     &   Est.    & &     S.E     &   Est.    & &     S.E  \\ \toprule
%         (Intercept) &   1.01    &**&    0.351   &   0.53    & & 0.416   &   0.79    &*& 0.321   &   0.50    & &  0.384   \\
%         Openness    &   -0.06   &  &    0.088   &   -0.07  & &  0.088   &   -0.15   &.& 0.081   &   -0.16   &*& 0.081 \\ \midrule
%         Condition (Inacc)    &   -1.12   &***&    0.124   &   -0.33  & &  0.393   &   -0.91   &***& 0.113   &   -0.33   & & 0.363 \\
%         AI Literacy    &   -0.01   &  &    0.013   &   0.024  & &  0.022   &   0.01   &  & 0.012   &   0.03   & & 0.020 \\ 
%         Condition (Inacc) X AI Literacy    &      &  &       &   -0.06  &*&  0.026   &      &   &    &   -0.03   & & 0.024 \\ 
%          &   \multicolumn{3}{c}{Adj. $R^2$=0.296***} &   \multicolumn{3}{c}{Adj. $R^2$=0.309***}     &   \multicolumn{3}{c}{Adj. $R^2$=0.260***}     &   \multicolumn{3}{c}{Adj. $R^2$=0.264***} \\ 
%         \bottomrule
%     \end{tabular}

%     \vspace{3mm}
    
%     \setlength{\tabcolsep}{1em}
%     \renewcommand{\arraystretch}{1.2}
%     \begin{tabular}{lllllllllllll}
%         &   \multicolumn{6}{c}{\textbf{Anthropomorphism}}   &   \multicolumn{6}{c}{\textbf{Likeability}}  \\ 
%         &   \multicolumn{3}{c}{\textbf{3a. Base}}   &    \multicolumn{3}{c}{\textbf{3b. Base + Interaction}}    &   \multicolumn{3}{c}{\textbf{4a. Base}}   &    \multicolumn{3}{c}{\textbf{4b. Base + Interaction}}  \\ 
%         &   Est.    & &     S.E     &   Est.    & &     S.E     &   Est.    & &     S.E     &   Est.    & &     S.E  \\ \toprule
%         (Intercept) &   0.54    &*&    0.256   &   0.64    &*& 0.307   &   0.81    &**& 0.296   &   0.63    &.&  0.354   \\
%         Openness &   -0.08    & &    0.064   &   -0.08    & & 0.065   &   -0.17    &*& 0.074   &   -0.17    &*&  0.075   \\ \midrule
%         Condition (Inacc) &   -0.50    &***&    0.090   &   -0.66    &*& 0.290   &   -0.59    &***& 0.104   &   -0.29    & &  0.334   \\
%         AI Literacy &   0.00    & &    0.009   &   -0.01    & & 0.016   &   0.00    & & 0.011   &   0.017    & &  0.018   \\
%         Condition (Inacc) X AI Literacy &       & &       &   0.01    & & 0.019   &       & &    &   -0.02    & &  0.022   \\
%         &   \multicolumn{3}{c}{Adj. $R^2$=0.137***} &   \multicolumn{3}{c}{Adj. $R^2$=0.134***}     &   \multicolumn{3}{c}{Adj. $R^2$=0.160***}     &   \multicolumn{3}{c}{Adj. $R^2$=0.159***} \\ 
%         \bottomrule
%     \end{tabular}
%     \label{tab:moderation}
% \end{table}

% \begin{figure}
%     \centering
%         \begin{subfigure}[b]{0.3\textwidth}
%             \centering
%             \includegraphics[width=\textwidth]{source/figures/post_steps_trust.pdf}
%             \caption{}
%             \label{fig:trust_steps}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}[b]{0.3\textwidth}
%             \centering
%             \includegraphics[width=\textwidth]{source/figures/post_human_trust.pdf}
%             \caption{}
%             \label{fig:trust_human}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}[b]{0.3\textwidth}
%             \centering
%             \includegraphics[width=\textwidth]{source/figures/post_use_trust.pdf}
%             \caption{}
%             \label{fig:trust_use}
%         \end{subfigure}
%     \caption{Post-hoc analysis with three general AI literacy sub-dimensions: AI steps knowledge, human actors in AI knowledge, AI usage experience. A significant effect between each literacy sub-dimension and condition were found in all three linear regression models with changes in overall trust as the outcome variable. All three models controlled for Openness personality dimension. We also found a significant main effect of AI usage experience on students' changes in overall trust of SAMI after encountering AI misrepresentation.}
%     \label{fig:post-hoc_analysis}
% \end{figure}

We then conducted post-hoc analysis to explore which specific dimensions of general AI literacy play an effect on students' changes in their overall trust in AI after encountering AI mistakes. We set up five linear regression models with students' changes in overall trust in SAMI as the outcome variable and included an effect of condition, each of the five AI literacy dimensions from the general AI literacy scale, and an interaction effect between condition and each AI literacy dimension. 
% \footnote{The general AI literacy scale measures five dimensions of general AI literacy:~\textit{AI technology knowledge}, which measures people's knowledge of what makes AI distinct from other technology and the role of AI in human-AI interaction;~\textit{Human actors in AI knowledge}, which measures people's knowledge of the role of human actors in human-AI interaction;~\textit{AI steps knowledge}, which measures people's general knowledge about AI's input, processing, and output, and each step's impact on AI performance;~\textit{AI usage experience}, which measures people's experience in using and interacting with different AI in their daily lives;~\textit{AI design experience}, which measures people's experience in designing and developing AI models and/or AI-driven products. }. 
We controlled for the Openness personality dimension in all five models. We plotted out the interaction effect of each model (Fig.~\ref{fig:post-hoc_analysis} in Appendix~\ref{appendix:s2posthoc}) and we found a significant interaction effect between condition and students'~\textit{AI steps knowledge} (Est. = -0.23, S.E = 0.101, p < 0.05) on changes in students' overall trust in SAMI after encountering AI misrepresentations. This suggests that students with more general knowledge about AI's input, processing, and output are more likely to change their overall trust in AI after encountering AI misrepresentations. We also found a significant interaction effect between condition and students'~\textit{human actors in AI knowledge} (Est.=-0.22, S.E=-.111, p<0.05) on changes in students' overall trust in AI after encountering AI misrepresentations. Our result suggests that students with more knowledge of human involvement in the design and development of AI are more likely to change their overall trust in AI after encountering AI misrepresentations. Finally, we found a significant interaction effect between condition and students'~\textit{AI usage experience} (Est.=-0.32, S.E=0.112, p <0.01) and a significant effect of students'~\textit{AI usage experience} (Est.=0.19, S.E=0.086, p < 0.05) on changes in students overall trust in SAMI after encountering AI misrepresentations. This shows that students with more experience interacting and using different AI in their daily lives are more likely to change their overall trust in AI after encountering AI misrepresentations. 

% The general AI literacy scale measures five dimensions of general AI literacy:~\textit{AI technology knowledge}, which measures participants' knowledge regarding what makes AI distinct from other technology and the role of AI in human-AI interaction;~\textit{Human actors in AI knowledge}, which measures participants' knowledge of the role of human actors in human-AI interaction;~\textit{AI steps knowledge}, which measures participants' general knowledge about AI's input, processing, and output, and each step's impact on AI performance;~\textit{AI usage experience}, which measures participants' experience in using and interacting with different types of AI in their daily lives;~\textit{AI design experience}, which measures participants' experience in designing and developing AI models and/or AI-driven products. 

% In our post-hoc analysis, we ran five linear regression models with students' changes in overall trust in SAMI as the outcome variable, and included an effect of condition, each AI literacy dimension, and an interaction effect between condition and each AI literacy dimension. We controlled for the Openness personality dimension in all five models. We plotted out the interaction effect of each model in supplementary materials. Among the five individual models, we found a significant interaction effect between condition and students'~\textit{AI steps knowledge} (Est. = -0.23, S.E = 0.101, p < 0.05) on changes in students' overall trust in SAMI after encountering AI misrepresentations.
% % plotted in Figure~\ref{fig:trust_steps}. 
% This suggests that compared to students with little general knowledge about AI's input, processing, and output, students with more~\textit{AI steps knowledge} are more likely to change their overall trust in AI after encountering AI misrepresentations. We also found a significant interaction effect between condition and students'~\textit{human actors in AI knowledge} (Est.=-0.22, S.E=-.111, p<0.05) on changes in students' overall trust in AI after encountering AI misrepresentations 
% % (see Figure~\ref{fig:trust_human}). 
% Our result suggests that students with more knowledge of human involvement in the design and development of AI are more likely to change their overall trust in AI after encountering AI misrepresentations, compared to those with little~\textit{knowledge about human actors in AI}. Finally, we found a significant interaction effect between condition and students'~\textit{AI usage experience} (Est.=-0.32, S.E=0.112, p <0.01) 
% % (shown in Figure~\ref{fig:trust_use}) 
% and a significant effect of students'~\textit{AI usage experience} (Est.=0.19, S.E=0.086, p < 0.05) on changes in students overall trust in SAMI after encountering AI misrepresentations. This shows that students with more experience interacting and using different AI in their daily lives are more likely to change their overall trust in AI after encountering AI misrepresentations, compared to students with little~\textit{AI usage experience}. 


==> source/6discussion.tex <==
\section{Discussion}
Through our mixed-methods approach, we offered insights on how people's existing and newly acquired knowledge of AI are highly connected to people's reactions and perceptions of AI after encountering AI misrepresentations. Specifically, we identified three rationales that participants adopted to interpret AI (mis)representations, reflecting participants' knowledge acquired from viewing AI outputs: AI works like a machine, a human, and/or magic. We found these rationales to be highly connected to participants' reactions of over-trusting, rationalizing, and forgiving of AI misrepresentations. Building on top of prior work that has suggested people's tendency of over-trusting and viewing AI as an authority~\cite{kapania2022because,warshaw2015can,hollis2018being}, we highlighted that these reactions and perceptions still persisted, and even exacerbated, when people encountered AI misrepresentations. We also empirically established that people's existing AI knowledge, i.e., AI literacy, can significantly moderate changes in people's trust of the AI after encountering AI misrepresentations, highlighting the importance of taking into account of people's knowledge and characteristics when building trustworthy AI systems~\cite{chen2023machine,chen2023understanding,ehsan2020human,schoeffer2022there}. In this section, we further unpack how people navigate AI fallibilities through their evolving AI knowledge. We then discuss implications for designing responsible mitigation and repair strategies by considering people's AI knowledge when AI fails. 

% In this section, we discuss the three rationales by situating them with recent literature on AI folk theories and machine heuristics, highlighting that this set of rationales provides a unifying lens to explain people's beliefs of AI from a holistic view. We then put these rationales into practice and provide implications for building and designing adaptable AI recovery strategies based on these three rationales. 

% We empirically confirmed algorithm aversion, where people can quickly lost trust in the algorithm outcome after encountering AI mistakes. We also contributed further findings that algorithm aversion could be moderated by the effect of AI literacy through our quant study; it could also be affected by how much participants could interpret AI's predictions. Setting proper expectations therefore is not enough. 

% Implication for designing XAI when AI literacy, especially usage experience should be taken into account of, besides just providing an explanation. Delicate balance to strike in terms of mistrust and over-trust. 

% - Defining rationales
% - Distinguish rationales from all the heuristics
% - Explaining rationale switching, one aspect of how it occurs, application of the lens, to 

\subsection{Navigating AI Fallabilities Through Evolving AI Knowledge}
Our findings suggest that when facing AI mistakes such as AI misrepresentations, people acquire new knowledge about the AI, which could be consistent or inconsistent with their existing AI knowledge, prompting them to adopt a dominant rationale to explain such AI behaviors. Contrary to prior work that uses fixed heuristics to explain people's perceptions and reactions to AI systems~\cite{sundar2019machine,sundar2020rise,nass1994computers}, our findings suggest that people are constantly re-framing their perceptions
% people's perceptions are constantly changing 
as they were presented with or discovered new information about the AI~\cite{devito2017platforms}. In Study 1, participants rarely stuck to one rationale about SAMI throughout, but kept navigating between different rationales, sometimes within a matter of seconds, as new information occurred to them. This suggests the instinctive nature of people's rationales~\cite{chen2023machine,chen2023understanding}--- we noticed that people rarely paused and reflected on their mental models~\cite{gero2020mental,wang2021towards} or folk theories~\cite{devito2017platforms,eslami2016first} of the AI before reacting to the AI output. This process of adopting various rationales, or concepts, to reconcile newly acquired knowledge with existing knowledge is similar to what was described as ``conceptual change''~\cite{ozdemir2007overview,chi1994things} in learning sciences, suggesting that people's re-framing of their perceptions
% people's perception changes 
could be viewed as an evolving learning process about AI~\cite{wang2021towards}.

We note that people's rationales are often bounded by their existing AI knowledge, i.e., AI literacy~\cite{long2020ai,druga2017hey}. In Study 1, we observed that participants who self-reported as ``Expert'' in tech proficiency were more likely to adopt the machine rationale, whereas participants who self-reported as ``Intermediate'' were more likely to adopt the human rationale. Some participants also constantly referred back to their lack of AI literacy when interpreting SAMI's outputs, prompting them to adopt the magic rationale. Our findings also suggest that people's existing AI knowledge, like people's evolving rationales, are also subject to frequent changes. Our posthoc analysis showed that while dimensions such as AI steps knowledge and human actors in AI require formal or informal intentional learning about AI, people's AI usage experience is also a crucial dimension of AI literacy that could moderate changes in people's trust after encountering AI misrepresentation. This is also reflected in Study 1 where many participants mentioned their experience with ChatGPT when talking about their over-trust in SAMI and their magic rationale. This further emphasizes that people are constantly learning from their daily interactions with AI systems, which contributes to their evolving AI knowledge. 




% \subsection{Machine, Human, or Magic? A Unifying Lens to Explain People's Beliefs of AI}
% Based on our findings, we propose these three rationales as a unifying lens to understand people's beliefs and reactions to AI. These rationales share a similar function as people's mental models~\cite{wang2021towards,gero2020mental}, heuristics~\cite{sundar2019machine,sundar2020rise}, and folk theories about AI~\cite{devito2018people,liao2021crystal} in that it has explanatory, analytical, and potential predictive power to understand people's perceptions and reactions to AI. However, these rationales also expand beyond these existing theories and heuristics. While prior work on machine heuristics~\cite{sundar2019machine,sundar2020rise}, folk theories~\cite{liao2021crystal,devito2017platforms}, and the CASA paradigm~\cite{nass1994computers} provided valuable insights into people's beliefs, perceptions, and reactions to AI systems, in our studies, we found each of them to only be able to partially explain the range of perceptions and reactions after people encountered AI misrepresentations, and less than sufficient in explaining the significant changes in people's perceptions and reactions after encountering AI misrepresentations.

% For instance, while machine heuristic has largely been used to explain people's over-trust in AI~\cite{sundar2019machine,sundar2020rise}, our data suggests that people often over-trusted AI without even thinking about the fact that it's a machine with basic input-processing-output mechanism--- they more often could not identify a connection between the input and AI output, and therefore opted in the magic rationale to imply that ``because it's an AI and it just somehow worked.'' Another example would be our observation of people showing concerns about AI misrepresentations in team matching given that AI might spread inaccurate impressions of them, but then immediately dismissing their own concerns within seconds after realizing ``it's just an AI'' [machine rationale]. We found this type of extreme switch in people's attitudes difficult to be explained with the existing theories, given that most of these theories often treat people's perceptions of AI as fixed states. 

% The main characteristics of these three rationales as a unifying lens is that they are not fixed states, but states that are constantly changing as participants were presented with or discovered new information about the AI, or even just immediately realized something they already knew about the AI. In our study sessions, we found that participants rarely stuck to one rationale about SAMI throughout the session, but kept switching between the three rationales to reconcile new incoming information about the AI with their existing knowledge about the AI. This switching happened frequently and swiftly, sometimes within a matter of seconds, as things occurred to them. This suggested the instinctive nature of people's rationales--- we noticed that people rarely paused and reflected on their mental models of the AI before reacting to the AI. The malleability characteristics of this set of rationales are consistent with~\citeauthor{devito2017platforms}[2017]'s findings on people's folk theories about algorithm-driven social media feeds. However, building on top of their work, we additionally outlined the three specific rationales to provide explanatory power about people's perceptions and reactions of AI.

% To summarize, leveraging this set of rationales as a unifying lens provides explanatory and analytical power to help researchers not only make sense of people's perceptions, beliefs and reactions of AI, but also provides explanations and an analytical framework to understand people's sudden changes in their perceptions and reactions of AI, especially after encountering AI mistakes. However, the associations between these rationales and people's specific reactions and behaviors towards AI will need to be further examined for this lens to provide predictive power of people's behaviors. 


% For instance, P28 over-trusted SAMI even though she recognized SAMI made inaccurate inferences about her. However, she was still concerned that SAMI might be right and this was how her friends saw her from the outside. She then continued by saying SAMI was an AI and it's really smart, and it should know about her personality traits. Machine heuristics could be leveraged to explain P28's thoughts about AI being smart, which could fit in with machine heuristics logic about people perceiving machines as logical and emotionless, hence her over-trust in SAMI's inaccurate inferences; however, machine heuristics was not sufficient in explaining P28 treating SAMI's inferences as an outside human perspective on her personalities. 


% Building upon prior knowledge about machine heuristics~\cite{sundar2020rise} and folk theories~\cite{devito2017platforms,devito2018people,liao2021crystal,karizat2021algorithmic}, we proposed these three rationales as a unifying lens to look at people's beliefs and understandings of AI systems before and after they encountered AI mistakes. While prior work on folk theories of AI algorithms has provided much insights into how people perceived and interpreted the AI~\cite{liao2021crystal,devito2017platforms,karizat2021algorithmic}, these folk theories were distilled from people's interactions with matured AI products with high accuracy, and thus may not cover or explain people's changes in their beliefs and perceptions after encountering AI misrepresentations. While machine heuristics~\cite{sundar2020rise} has proven to be highly effective in explaining people's overtrust and overreliance on AI, we found it difficult to leverage machine heuristics to explain other reactions participants had about AI such as dismissing concerns about AI misrepresentations, or explaining SAMI's inference-making process by attributing perceived human inference-making process. These three rationales therefore provides a unifying lens to understand and interpret people's beliefs and reactions to AI systems with varying levels of accuracy.


% Based on our findings, we proposed a unifying lens to understand people's beliefs and interpretations of AI through three rationales: AI works like a machine, AI works like humans, and AI works like magic. Consistent with prior literature on users' mental models about AI~\cite{wang2021towards,gero2020mental}, we found that these rationales guided participants' reactions and attitudes of the AI after encountering AI misrepresentations: participants in our study over-trusted AI misrepresentations about them based on their rationale that AI is powerful and ``AI works like magic''; participants rationalized and ``justified'' AI's misrepresentations because ``AI works like a machine'' that relied on quality input; participants showed concerns about AI misrepresentations because ``AI works like a human'' that could generate harsh language and spread negative impressions about them; yet participants also showed a lack of concern about AI misrepresentations because ``AI works like a machine'' and could not take into account people's feelings possibly getting hurt by it, or drew valid inferences about human characteristics. 

% These three rationales are not fixed, but fluid and malleable as participants were presented with or discovered new information about the AI, similar to what \citeauthor{devito2017platforms} have found about people's folk theories about social media feeds~\cite{devito2017platforms}. In our study sessions, we found that participants rarely stuck to one rationale about SAMI throughout the session, but kept switching between the three rationales to reconcile new incoming information about the AI with their existing knowledge about the AI. This switching happened frequently, sometimes within a matter of seconds, as things occurred to them. For instance, participants described their concerns about AI misrepresentations when they were following the ``AI works like a human'' rationale, but then immediately dismissed their concerns when they switched to the ``AI works like a machine'' rationale when they realized ``it's just an AI.'' 

% Combining with our findings in Study 2, we identified AI literacy as a core factor that influenced participants' disposition to rationale switching when interacting with AI. Our findings from study 2 suggested that AI literacy was a significant moderator on changes in people's overall trust in AI after encountering AI misrepresentations. We also noticed in study 1 that the level of connections participants were able to make between the self-introduction paragraph and SAMI's inferences could also trigger their rationale switching--- when participants couldn't make sense of how SAMI drew certain inferences from the introduction paragraph, many participants opted to switch to the ``AI works like magic'' rationale. 

% We also want to highlight one of the rationales ``AI works like magic'', which we have not come across in existing work. 

% While prior work has suggested people identified AI systems as more capable and having more expertise than them in recognizing their own personalities and emotions when shown accurate personality inferences~\cite{warshaw2015can,hollis2018being}, we were surprised to find that this phenomenon still persisted when participants in our study were shown inaccurate personality inferences--- many of them continued to trust and even rationalize these inaccurate inferences about them. Falling into the trap of cognitive biases such as the Barnum effect is common for people, yet when it comes to AI-generated inferences that are ambiguous and implicit, people appeared to be more likely to blindly trust AI's inferences about them, based on their rationale that ``AI works like magic.'' 



% - Identifying rationales can help change interactions
% - People with different AI literacy needs to be distinguished, interventions needs to be distinguished, rationale helps inform rationales. Interventions need to be different bc they might have different rationales. While literacy and rationales could be associated, outside of scope of this study, encourage future work to look into it. 
% - Predicting rationale using linguistic cues. 

\subsection{Designing Responsible Mitigation by Considering People's AI Knowledge} 
% Our findings provided evidence to the ongoing discourse about whether AI failures could negatively impact people's perceptions of AI~\cite{honig2018understanding,salem2015would,mirnig2017err,dietvorst2015algorithm}--- we found people's overall trust and social perceptions of the AI (perceived intelligence, anthropomorphism, and likeability) all significantly decreased after encountering AI misrepresentations. Further, our analysis in Study 2 showed that people with more general knowledge about AI are susceptible to changes in overall trust of AI after encountering AI misrepresentations; yet people with less general knowledge about AI had less changes in their overall trust of AI after encountering AI misrepresentations. Posthoc analysis showed people's knowledge about general AI input-processing-output, knowledge of human actors involvement in AI design and development, and their daily usage experience of different types of AI were significant moderators, but not advanced technical knowledge or experience with AI design and development. While we did not look into the relationships between changes in perceptions and people's rationale switch behaviors, AI literacy present itself as a promising factor used to predict changes in perceptions or even people's rationale switch behaviors. 

While much of prior work has shown people's tendency to view AI as an authority~\cite{kapania2022because,warshaw2015can} and to overtrust AI-generated responses~\cite{warshaw2015can,gou2014knowme,hollis2018being}, our work, focusing on the scenario where AI makes mistakes, demonstrated that people would still over-trust, forgive, and even rationalize AI's obvious misjudgment in their most personal characteristics. We consider these responses to be highly connected to the rationale people adopted at the time, suggesting that some aspects of certain rationales could be harmful and even dangerous when generalized. This was illustrated by P28's reactions when she clearly recognized that SAMI's personality inferences about her were inaccurate, yet her perceived lack of AI knowledge prompted her to adopt the ``AI works like magic'' rationale and believed SAMI's misrepresentations could be true. This caused confusion, mental discomfort, and even self-doubt for P28. We therefore urge designers and developers of AI systems and algorithms that could infer people's personal traits such as personalities, emotions, preferences, to be aware and cautious of the potential harm to the user when such AI systems exhibit ``gaslighting'' behaviors, and design appropriate mitigation strategies to mitigate the potential harms. Based on our findings, we propose to incorporate people's evolving AI knowledge when designing mitigation strategies when AI fails. 

Existing repair and mitigation strategies mostly focus on adding social elements such as politeness, apologizing, or setting user expectations early in the interactions~\cite{honig2018understanding,lee2010gracefully,mahmood2022owning}. These strategies, without considering users' evolving AI knowledge, could risk eliciting undesired outcomes such as reinforcing people's social behaviors towards AI~\cite{nass1994computers} or confusing the users about AI's true capabilities as they learn. Echoing with prior work that people's beliefs and intuitions should be taken into consideration when designing AI explanations~\cite{miller2019explanation,liao2021human,ehsan2020human,long2020ai} and repair strategies~\cite{ashktorab2019resilient,chen2023understanding}, we provided a specific set of rationales and encourage future work to explore techniques that could allow automatic identifications of users' rationales in real-time. One mitigation strategy could be to provide explanations tailored to the specific rationale that people adopted at the time. For instance, if a user adopted the magic rationale, the AI could provide explanations to nudge the user to adopt the machine rationale to reduce overreliance. 

Additionally, people's existing AI knowledge, i.e., AI literacy~\cite{long2020ai,druga2017hey}, could be leveraged to approximate the ``cost'' of an AI misrepresentation when providing customized mitigation strategies. Our study found that people with lower AI literacy were not affected much by their trust in AI after encountering AI misrepresentation. Given that they still trust the AI after the AI erred, they might not provide any feedback, which could give the AI developers a false sense that the AI was working fine, leading to long-term repercussions. By contrast, while more AI literacy in a user can seem favorable, our study showed that it could lead to more extreme changes in trust perceptions in AI after AI misrepresentations. People with more AI literacy might abandon the system after encountering AI failures, which makes recovery non-trivial. By considering AI literacy as a factor, we have an opportunity to consider different repair strategies by estimating the different effects of AI misrepresentations for people with varying AI literacy levels.

% However, while the magnitude of each rationale might vary since these rationales could co-occur together, rationale-based approach could significantly reduce the dimensions of user perceptions down to three: machine, human, magic. By identifying each rationale and the magnitude of each rationale, users' attitudes and behaviors could be predicted in real time once certain associations between user attitudes and rationale are established. For example, participants employed the ``AI works like magic'' rationale might have a tendency to blindly trust AI; participants employed the ``AI works like a machine'' rationale might have a tendency to rationalize and justify AI mistakes. Rationale-based approach could also enable timely nudges towards the participants when they over-estimated AI's capabilities. For instance, when users overly anthropomorphized AI and scored high on the ``AI works like a human'' rationale, nudging the users to move towards the ``AI works like machine'' rationale would be appropriate to avoid further anthropomophization that could lead to serious consequences~\cite{blut2021understanding}. Identifying how users think of AI in terms of rationales in real time would also move us one step closer to the ultimate vision of Mutual Theory of Mind in human-AI interaction~\cite{wang2021towards}.

% Our studies provided some directions towards automatically identifying people's rationales about AI. In our study, we qualitatively distilled certain associations between people's rationales and their reactions to AI. We encourage future research to quantitatively validate these associations to develop rationale-based approaches in predicting user attitudes and behaviors towards AI. We also want to highlight the role of AI literacy in significantly moderating the effect of changes in people's overall trust in SAMI after encountering AI misrepresentations. This suggests that AI literacy could be a crucial factor in predicting people's rationale-switch behaviors. Given that people's language used when describing how SAMI works gave us hints about the rationales they employed, we also encourage future research to consider linguistic cues and certain key words to be potentially promising factors that could be used to predict people's rationales about AI. 

% Our findings provided evidence to the ongoing discourse about whether AI failures could negatively impact people's perceptions of AI~\cite{honig2018understanding,salem2015would,mirnig2017err,dietvorst2015algorithm}--- we found people's overall trust and social perceptions of the AI (perceived intelligence, anthropomorphism, and likeability) all significantly decreased after encountering AI misrepresentations. However, consistent with what we observed from Study 1, even though there was a decrease in overall trust for participants in the inaccurate group, most participants in the inaccurate condition did not change or changed slightly in terms of their overall trust in SAMI when they were shown intentionally inaccurate SAMI inferences (see~\ref{fig:density_trust}). \chelsea{<-- @vedant can you check me on this?} Given that AI literacy acted as a significant moderator in people's changes in overall trust after encountering AI misrepresentations, AI literacy could be leveraged as a key factor to predict people's rationale-switch behaviors, which are associated with people's reactions and attitudes such as over-trust and rationalizations. 


% - We observed how people's trust and social perceptions are significantly affected by encountering AI misrepresentations. People's reactions and perceptions are also based on three rationales. 
% - AI literacy and posthoc analysis. Automatically identifying the rationales?
% - Repair strategies and explanations should be tailored to user's state of mind after encountering AI misrepresentations. 
% - Current repair strategies focuses on expectations and AI's way of communication such as anthropomorphism, however not targeted at people's beliefs or perceptions of the AI after encountering mistakes. AI literacy plays a role in moderating the changes in trust, and should be taken into account when predicting people's state of mind after encountering AI misrepresentations.
% - We also echo with human-centered XAI community that explanations should consider people's beliefs and state of mind. This can also help achieve MToM in human-AI interactions. 






==> source/7conclusion.tex <==
\section{Limitations}
% While our work provides valuable insights and implications into people's AI knowledge in shaping their perceptions and reactions to AI misrepresentations, our work has limitations. 
Our work has some limitations. First, we only studied people's perception changes after encountering a one-time AI misrepresentation in a very short period of time. People's perceptions and rationale change behaviors could be more stable in the long run~\cite{wang2021towards}, and we encourage future research to replicate our studies in longer-term settings and contexts. Second, while we incorporated many relevant covariates in our models, other factors that were not modeled could impact people's perceptions of AI, e.g., people's attitudes towards specific types of AI. Third, all study participants in study 1 were recruited from a large public technical institute and, despite our efforts to target recruit participants from non-STEM disciplines, participants in study 1 might have more knowledge and exposure to AI technologies than average college students. All of our study participants were recruited from the U.S. and may only represent Western attitudes and perceptions of AI~\cite{kapania2022because}. Future studies should consider replicating our study in non-western regions to understand the cultural differences in changes in perception and reactions of AI after encountering AI mistakes.

\section{Conclusion}
We reported on semi-structured interviews (n=20) and a large survey experiment (n=198) with college students in the United States to understand their perceptions and reactions of AI after encountering personality misrepresentations in AI-facilitated team matching. Through the two studies, we highlighted the critical role of people's existing and newly acquired knowledge of AI in shaping people's reactions and perceptions of AI after encountering AI misrepresentations. We emphasized the ever-evolving nature of people's AI knowledge acquired from viewing AI outputs by pinpointing three rationales that people adopted to interpret AI (mis)representations: AI works like a machine, a human, and/or magic. These rationales are bounded by people's existing AI knowledge and are highly connected to people's tendency to over-trust, rationalize, forgive AI misrepresentations. We also found that people's existing AI knowledge, i.e., AI literacy, could significantly moderate changes in people's trust in AI after encountering AI misrepresentations. We discussed how people navigate AI fallibility through their evolving AI knowledge and provided implications for designing and developing responsible mitigation strategies that consider people's evolving AI knowledge to reduce potential harms when AI fails. 


% identify three rationales that people employed when interpreting the AI: AI works like a machine, AI works like a human, and AI works like magic. We found people over-trusted, rationalized, and expressed concerns and/or lack of concerns about AI misrepresentations, all of which could be explained by their rationales. By quantifying people's perceptions of AI, we found that encountering AI misrepresentations significantly lowered people's perceptions of AI, with AI literacy as a significant moderator in changes in people's overall trust in AI. Based on our findings, we proposed the three rationales as a unifying lens to understand and interpret people's beliefs, perceptions, and reactions of AI. We discuss implications for future design and development of ethical and resilient AI through automatic identifications of these three rationales.  

==> source/deleted.tex <==


% \subsection{People's Reactions and Perceptions of Faulty AI} 
% % Much research has been conducted to understand how people perceive AI agents differently after encountering AI failures, most of which had been done in the area of human-robot interaction. Prior work established that encountering robot failures would significantly lower people's perceptions of the robot~\cite{honig2018understanding} in terms of robots' trustworthiness~\cite{salem2015would,law2017wizard,roesler2020effect}, perceived intelligence~\cite{takayama2011expressing}, perceived likeability~\cite{mirnig2017err}, anthropomorphism~\cite{salem2015would}, reliability~\cite{salem2015would}, and ease of use~\cite{de2023we}. However, some of these results were inconclusive given that other research has suggested that AI mistakes could be considered as a human-like characteristics, and therefore could make the interactions more engaging and natural, mitigating the potential negative effect AI mistakes might have on users' perceptions of the AI~\cite{honig2018understanding,buhrke2021making,mirnig2017err}. For instance,~\citeauthor{mirnig2017err} [2017] did not find a significant difference in perceived intelligence and anthropomorphism between participants who interacted with faulty robots vs. flawless robots~\cite{mirnig2017err}; studies also suggested that robot failures might make users' interaction experience more pleasurable~\cite{mirnig2017err,honig2018understanding,gompei2015robot} and more engaged~\cite{honig2018understanding,law2017wizard}. Some prior work has offered explanations that people's perception after encountering robot failures might be attributed to a number of factors such as types of failures, failure severity, or the nature of the task (e.g., formal workplace or social and personal)~\cite{sarkar2017effects,honig2018understanding,rossi2017timing}. Therefore, it is important to examine how people's perceptions changed after encountering AI mistakes in different context to better inform the human-centered design of AI's repair and recovery strategies. 

% % There is also a growing body of research in HCI focused on studying people's reactions and attitudes of towards AI algorithms such as recommendation algorithms, with ``trust'' as the core concept of interest. Much research in this area suggested that people had a tendency to overtrust AI~\cite{oh2022you,banas2022machine,kapania2022because} and to attribute more credibility to AI~\cite{kapania2022because,edwards2016robots} comparing to human agents--- some even pointed out that AI was considered as an authority figure that could influence people's behaviors without needing to provide adequate evidence~\cite{kapania2022because}. In their interview study on people's perceptions and attitudes of AI in India,~\citeauthor{kapania2022because} [2022] found that people seemed to have a high tolerence of AI failures, with some displaying tendencies of forgiving and justifying AI misfires, or even blame themselves or others for AI's mishaps~\cite{kapania2022because}. Many researchers attributed this tendency to overtrust AI to people's machine heuristics~\cite{sundar2020rise}: the belief that machines are objective, emotionless, and logical entities without feelings, therefore more trustworthy comparing to humans~\cite{sundar2020rise}. 

% % However, only a few work has empirically studied people's reactions and attitudes towards AI mistakes, and suggested additional, sometimes contradictory findings. For example, instead of overtly positive view and reliance on AI,~\citeauthor{hsu2021attitudes} [2021] found that students perceived AI autograders as unfair and harmful due to their over-estimation of the AI's error rate~\cite{hsu2021attitudes}. While~\citeauthor{oh2022you} [2022] corroborated with findings from prior literature that people tended to have greater trust and more positive attitudes towards machine-generated recommendations comparing to human-generated recommendations, they also found that people's trust and general attitudes declined quickly after users saw machines made mistakes (also known as the phenomenon of algorithm aversion~\cite{dietvorst2015algorithm}). This suggested that multiple heuristics could exist and interact together to shape people's perceptions and attitudes towards AI after encountering AI mistakes. 


% % \cite{hsu2021attitudes}: understanding students' attitudes, knowledge, and perception. Misalignments between students' folk theories about the autograder and how it actually worked. Perceived the autograder as unfair and harmful due to incorrect estimation.

% % \cite{oh2022you}: people showed more positive attitude toward a machine recommender than a human recommender. Machine heuristic: the higher the users perceive the rec as machine, the more positive attitudes. Automation bias induces people to adhere to automated decision authorities. Over-credence on recommendation algorithm. 

% % \cite{dietvorst2015algorithm}: algorithm aversion: people quickly lose confidence in algorithm than human forecasters after seeing them make the same mistake. 

% % \cite{banas2022machine}: Second, heuristic preference in machines and crowds matters more when the corresponding fact-checking agent labels a claim as true rather than false; this result is consistent with the idea that people are more tolerant of agents incorrectly fact-checking a story as true (false positives) than they are for the reverse when a story is incorrectly marked as false (false negatives). Third, system transparency explanations do not appear to interact with heuristics and agents’ assessments to affect veracity judgments. Overall, these results provide a nuanced understanding of how people rely on AI and human agents’ judgments and their own heuristic biases to make decisions about the veracity of truth-ambiguous information.

% % \cite{milani2023navigates}: assessments of human likeness are influenced by stereotyped beliefs about AI capabilities. Different people have different interpretations of what is human-like behavior. 

% % \cite{kapania2022because}: case of AI authority: forgiveness, self-blame. High tolerence for system misfires. Inclination to forgive or justify wrong decisions or incorrect recommendations. Blamed themselves for receiving an adverse outcome. View AI as machines, emotionless, logical entities. 

% % \cite{edwards2016robots}: teacher as robot was perceived as most credible. Machines are perceived as more objective, less capable of feeling and relating. 

% % \cite{wenzel2023can}: failed automatic speech recognition could lead to higher self-consciousness, lower marginalized groups' self-esteem and positive affect, less favorable ratings of the technology. 


% % - Trust and Machine Heuristic, view AI as an authority. Algorithm aversion -> transparency and XAI


% \subsection{Interacting with Hyper-Personalized AI Systems}
% % With the advancement of algorithms to detect and profile people's personal traits such as their emotions~\cite{wang2020sensing,disalvo2022reading,hollis2018being} and personality characteristics~\cite{gou2014knowme,warshaw2015can,liao2021crystal}, there has been some work conducted in HCI to understand people's reactions and concerns about this type of hyper-personalized AI systems. Prior work found that most users found their AI-generated personality profiles to be ``creepily accurate''~\cite{gou2014knowme,warshaw2015can,liao2021crystal,kim2020understanding}, which was cited as evidence in early studies as proof for feasibility and accuracy of personality recognition algorithms~\cite{gou2014knowme}. However, later qualitative research showed that, even though AI-generated personality profiles are about the users themselves, many users considered AI as an ``expert'' and better than them at recognizing their personalities and/or emotions~\cite{warshaw2015can,hollis2018being}:~\citeauthor{warshaw2015can} found that people felt unqualified to modify their personality profile generated by automated personality recognition algorithm due to their over-trust in the ``expert'' algorithm;~\citeauthor{hollis2018being} echoed this finding and added further that some users even overrode their personal judgements about their emotions, and believed that the AI algorithm was capable of identifying their ``hidden self'' and had privileged information about their emotions. 

% % Despite people's trust in AI-generated profiles about them, when it comes to sharing these AI-generated emotion or personality profiles about them, prior research identified a somewhat contradictory attitudes and opinions. Some suggested that users still wanted control over modifying their profile and traits before sharing due to concerns over others' misinterpretations of AI-inferred traits about them~\cite{gou2014knowme}; however, others have found that users felt compelled to share despite their reservations about sharing given that they wouldn't want others to think they had something to hide~\cite{warshaw2015can}.

% % To understand people's reasoning behind this myriad of attitudes and reactions,~\citeauthor{liao2021crystal} [2021] conducted qualitative interviews to pinpoint people's folk theories about automated personality recognition systems. Consistent with prior work on people's folk theories and beliefs about AI algorithms~\cite{eslami2015always,eslami2016first,devito2018people}, they found that people's reactions and attitudes were largely based on people's folk theories; for example, people with limited folk theories about the data source, data scope, and personalization of output about the AI algorithm allowed them to dismiss AI's personality inferences as less threatening~\cite{liao2021crystal}.~\citeauthor{kim2020understanding}[2020] further added that factors such as the data driven aspect of the system, users' self-perception of their own personality, and the ambiguity around how the system works could all influence people's trust in the result of AI-generated personality inferences. 


% % \cite{gou2014knowme}: two-part study with 256 participants. Showed there is a feasibility of deriving personality traits from social media. Over 61.5\% users are wiling to share their derived traits in the workplace and various factors (what to share, whom to share, and when to share) could influence their sharing preferences. Participants consider it as very personal information. Desire of system transparency on system usage and function. Highlighted two user concerns: others' misinterpretation of the user's inferred personal triats, and users wanting control to modify their profile and traits. 

% % \cite{warshaw2015can}: Qualitative study of people's reactions to a working hyper-personal analytics system. Our results reveal a paradox. Participants found their personal traits profiles creepily accurate and did not like sharing them in many situations. However, they felt pressured by the social risks of not sharing and showed signs of learned helplessness, leading them to share despite their misgivings. Further they felt unqualified to significantly moify their profile contents due to a surprising trust in the expert algorithm. 

% % \cite{hollis2018being}: we explore how people construe algorithmic interpretations of emotional data in personal informatics systems. Users still deferred to feedback and their perceived emotions were significantly influenced by feedback frames. Some users overrode personal judgments, believing the system had access to privileged info about their emotions. Risks of users trusting systems that seemingly unlock hidden aspects of the self.  

% % \cite{kim2020understanding}: participants' trust in results was affected by the following factors: (1) data driven aspect of the system, (2) self-perception of their own personality, and (3) ambiguity around how the system works. 

% % \cite{liao2021crystal}: this study examines how people construct ``snap'' folk theories about the ways personality algorithms operate as well as how they react when shown their outputs. Through qualitative interviews (n = 37) with people after being presented with their own profile, this study identifies a series of folk theories that people came up with to explain the personality algorithm across four dimensions (data source, scope, collection process, and outputs). In addition, this study examined how those folk theories contributed to certain reactions, fears, and justifications people had about the algorithm. Personalization of output: astrology to omniscience. The limited folk theories about... alowed people to dismiss it as less threatening. People's reactions depends on the kind of folk theories they formed (limited to advanced). Worried issues arising from inaccuracy. People blame themselves about data source

% % \cite{devito2018people}: form folk theory based on endogenous info (originates with the platform itself) and exogenous info: originate outside the platform. Folk theories are malleable. Show that the relationship between audience and self is no longer direct, as self-presentation used to be like described by Goffman. Web skills are related to people's folk theories and information source that they seek (high web skill tend to seek endogenous info)



% \subsection{AI-Facilitated Impressions in Human Community}
% % - People's relationships and perceptions of each other can now be mediated through AI algorithms.Folk theories and self-presentations. ~\cite{eslami2015always,eslami2016first}
% % AI-mediated social interactions such as online dating algorithms. 

% % - AI-mediated communication.

% % - But none of these examined AI-mediated impressions in the context of team-matching. This is a formal and relatively professional context and setting, yet based on people's most personal traits and characteristics. 

% % People's self-perceptions and relationships with others can be influenced and mediated by AI algorithms. 

% Our daily interactions and communications are heavily mediated through AI algorithms nowadays. As~\citeauthor{devito2018people} has pointed out in managing AI-mediated impressions in human communities, the relationship between ourselves and the audience are no longer as direct as~\citeauthor{goffman2016presentation} described. Much research has been done to understand and explore people's practices of managing their impressions through social media platforms that are powered by AI algorithms~\cite{karizat2021algorithmic,devito2017platforms,eslami2015always,eslami2016first}. This body of literature has suggested that people not only leverage platform affordances and their folk theories of the platform algorithms to build their self-presentations on the platforms~\cite{devito2017platforms,karizat2021algorithmic}, but also perceive of others and their relationships to others based on algorithm behaviors~\cite{eslami2015always,eslami2016first}. For instance, in their investigation of people's understanding of Facebook recommendation algorithms,~\citeauthor{eslami2015always} found that people formed misperceptions about their friends whose posts never showed up in their feed due to lack of understanding of the recommendation algorithm, which led them to make inferences about their relationships with that person. In the age of AI-mediated interactions, we have begun to see ourselves and others through the filtered lens of algorithms, which unfortunately often presented as a black box to people.

% The burgeoning area of AI-Mediated Communication (AI-MC)~\cite{hancock2020ai}, which referred to communications that are augmented, optimized, or generated by AI, has also offered implications of how AI-facilitated impressions could influence people's interpersonal communications and dynamics. Prior work has suggested that self-presentations or impressions, when knowingly augmented by AI, can decrease its perceived trustworthiness~\cite{jakesch2019ai} and undermine social attractions between people~\cite{mieczkowski2021ai}. However, some work also pointed out that AI could be perceived as having agency when facilitating human-human communications, leading people to transfer their impression of the AI to human~\cite{li2023impression} or having the AI acted as a moral crumble zone for humans to blame for communication breakdowns~\cite{hohenstein2020ai}.


% % \cite{karizat2021algorithmic}: participants changed their behaviors to shape their algorithmic identities to align with how they understood themselves. We argue the relationship between users' algorithmic folk theories and identity are consequential for social media platforms, as it impacts users' experiences, behaviors, sense of belonging, and perceived ability to be seen, heard, and feel valued by others as mediated through algorithmic systems. 

% % \cite{devito2018people}: form folk theory based on endogenous info (originates with the platform itself) and exogenous info: originate outside the platform. Folk theories are malleable. Show that the relationship between audience and self is no longer direct, as self-presentation used to be like described by Goffman. Web skills are related to people's folk theories and information source that they seek (high web skill tend to seek endogenous info)

% % \cite{devito2017platforms}: affordances of social media platforms that affect how people build their self-presentations. 

% % \cite{eslami2015always}: observing the output surprised some unaware participants by revealing misperceptions about their friends whose stories were not shown in the news feed at all. Use it to make inferences about their relationships. 

% % \cite{eslami2016first}: interviews revealed 10 folk theories of automated curation. 






% \section{Study 2: Examining the Impact of AI Misrepresentation on Students' Perception of AI}
% To examine the impact of AI misrepresentation on students' perception of AI (RQ3), we conducted a two-part longitudinal survey study on the Prolific crowdsourcing platform to solicit a larger and more diverse sample. We deployed study 2 by following a similar procedure as study 1 by first deploying a preliminary survey, then after a week, followed by a experiment survey to show participants SAMI's inferences and measured their perception changes of SAMI. We also made some minor revisions to the measurements based on our findings and observations from study 1. In study 2, we also further examined AI literacy as a possible moderating factor on students' changes in perceptions of AI after encountering AI misrepresentation. Specifically, study 2 aimed at answering two research questions to examine the impact of AI misrepresentation on students' perception of AI:

% \begin{table}[h]
% % \sffamily
% \centering
% % \footnotesize
% \vspace{-0.5em}
% \begin{tabular}{@{}l@{}p{0.92\columnwidth}@{}}
%     \textbf{RQ 3.1: } & What is the effect of AI misrepresentation on students' trust and social perceptions of the AI?  \\
%     \textbf{RQ 3.2: } & How does students' level of AI literacy moderate the effect of changes in students' perception of AI after encountering AI misrepresentation? \\
%     % \bottomrule
% \end{tabular}
% \vspace{-0.9em}
% \end{table}


% \subsection{Study 2 Study Design}
% \subsubsection{Study 2 Procedure} 
% Study 2 procedure largely remained the same as the study procedure of study 1, except that the semi-structured interview portion was removed in study 2 given that the aim of study 2 was to collect a large sample to quantitatively examine the impact of AI misrepresentation on students' perception of AI. 

% Similar to study 1, we first deployed a preliminary survey on the Prolific platform. Participants were told that the goal of this longitudinal study was to understand people's perception of a team-matching AI agent. In the preliminary survey, participants were asked to write a paragraph to introduce themselves to SAMI, filled out the 44-item Big Five personality test, a measurement of AI literacy and a measurement of their general attitudes toward AI. Participants then provided their demographic information, their level of study, major or background, as well as the number of team projects they have been involved with and their overall experience with their past team projects at school. All the participants were compensated with \$3 USD for their time after successfully completing the preliminary survey. The median completion time for the preliminary survey is about 11 min. 

% 250 prolific participants filled out our preliminary survey on Qualtrics. After manually checking through their survey responses one by one, we removed seven participants whose self-introduction paragraph were suspected to be generated by ChatGPT. We then wrote a python script to fabricate SAMI's inferences for the 243 remaining participants, following the same inference fabrication procedure and guideline that we described in section~\ref{fabrication}. All the fabricated inferences generated must follow the strict 60\% positive inference and 40\% negative inference ratio, which removed 21 participants in the participant pool given that these 21 participants' fabricated inferences were either too positive or too negative based on how they filled out their personality measurement. This resulted in 222 participants remaining and we invited all 222 participants back to participate in the second survey of study 2, which we refer to as experiment survey. Participants who were invited back to complete the experiment survey was randomly assigned to either the accurate condition or the inaccurate condition. Given our emphasis on AI misrepresentation, we assigned more participants to the ianccurate condition than the accurate condition--- we ended up assigning 157 participants to the inaccurate condition and 65 participants to the accurate condition. 

% The experiment survey, hosted on Qualtrics, was lightly modified based on the survey measurement used at the beginning of the user study session in study 1. After entering the survey, participants were first shown the two samples of self-introduction and SAMI's inferences, then prompted to answer their perceived accuracy of SAMI's inferences, the trust measurement, and the social perception measurement. The two samples were the same samples shown to the participants in study 1. We also randomized the order of the two samples being shown to the participants in the survey to remove potential order effect. Participants were then asked to enter their Prolific ID on another website to retrieve SAMI's inferences about them, and then fill out the same perception measurements. At the end of the survey, a debriefing form informing participants about the real purpose of the study and how SAMI's inferences were fabricated based on their personality survey answers were provided. Participants were compensated with \$3 USD for completing the experiment survey, and an extra \$4 USD bonus for completing both surveys. We received 211 responses (n=61 for accurate condition, n=151 for inaccurate condition) for the experiment survey. The median completion time for the experiment survey is about 12 min. 

% In our data processing of the experiment survey data, we removed ten participants' data given that they finished the experiment survey way too fast, in less than six minutes; we also removed an additional three participants' data given that there were obvious and prevalent contradictions in their survey responses. We ended up with 198 participants' data for experiment survey. 

% \subsubsection{Study 2 Measures}
% \chelsea{Study 1 Method will briefly mention the perception measures since the measures are now considered "probes."} 
% In this section, we describe the three scales that we used in the preliminary survey and the experiment survey that measured our moderator (AI literacy) and perception outcomes (trust, intelligence, anthropomorphism, and likeability). 

% \textbf{General AI Literacy Scale: } This 13-item scale was developed and validated by~\citeauthor{pinski2023ai} to measure general AI literacy, which they interpreted as ``humans' socio-technical competences regarding AI''~\cite{pinski2023ai}. This scale consists of five dimensions: AI technology knowledge, human actions in AI knowledge, AI steps knowledge, AI usage experience, and AI design experience. The responses were given to the 13 items on a five point Likert scale. Correlation test suggested that the five dimensions are highly inter-correlated, with correlation ranging from 0.31 to 0.73. To avoid inflating our model, we decided to use an overall literacy score that captures all these dimensions by taking the sum of the score for each dimension. 

% %%%%% explain the two significant moderator in post-hoc
% % This general AI literacy scale measures five dimensions of general AI literacy:~\textit{AI technology knowledge}, which measures participants' knowledge regarding what makes AI distinct from other technology and the role of AI in human-AI interaction;~\textit{Human actions in AI knowledge}, which measures participants' knowledge of the role of human actors in human-AI interaction; ~\textit{AI steps knowledge}, which measures participants' knowledge about AI's input, processing, and output and each step's impact on humans;~\textit{AI usage experience}, which measures participants' use experience with AI;~\textit{``AI design experience''}, which measures participants' experience in designing and developing AI models and/or AI-driven products. 

% % An overall AI literacy score was calculated by taking the sum of the score for each AI literacy dimension given that these dimensions are highly correlated with each other. We found these dimensions are highly inter-correlated, ranging from XX to XX. For the sake of simplicity in our model, we decided to use an overall literacy score that captures all these dimensions by taking the sum of them. \chelsea{@vedant I forgot why we decided to take the sum of all the AI lit dimensions... Was it because they were all highly correlated? And if so, how should I report the correlation here?}

% \textbf{Human-Computer Trust Scale:} We measured students' trust in SAMI by using the ``Human-Computer Trust Scale (HCTS)'' developed and validated by~\citeauthor{gulati2019design}. This scale consists of 12 statements that can be customized to the specific AI technology being studied, and responses were taken on a five-point Likert scale. This scale measures four dimensions of trust: perceived risk, benevolence, competence, and overall trust. Given that the scores for each of the dimensions were highly inter-correlated, with correlations ranging from -0.45 to 0.75, we took the score for overall trust to represent participants' trust in SAMI in our analysis. 

% % aims at measuring four dimensions of trust, and consists of 12 statements that can be customized to the AI technology studied and responses were taken on a five-point Likert scale with labels for ``Strongly Disagree'' (1), ``Neither Agree nor Disagree'' (3), ``Agree Strongly'' (5). 

% % We chose this scale given its focus on human-AI interaction and the multiple dimensions of trust it measures:~\textit{Perceived Risk, Benevolence, Competence, and Overall Trust.} ~\textit{Perceived risk} measures participants' assessment of the likelihood of certain incident happening with the use of certain technology and how concerned they would be with the consequences;~\textit{Benevolence} measures participants' perceptions of the helpfulness of the technology to help users achieve their goals;~\textit{Competence} measures participants' perception of whether the technology has all the features and functionalities to perform its intended tasks;~\textit{Overall Trust} measures participants' level of overall trust on the technology. 

% % A score for each dimension was calculated by taking the average of participants' reported score of statements that aimed at measuring the corresponding dimension. Given that the scores for each of the dimensions were highly inter-correlated (give a range OR .x with this dimension ``to avoid inflating the model'') \chelsea{@vedant how should I report the correlations here since there are multiple?}, we took the score for overall trust to represent participants' trust in SAMI in our analysis. 

% \textbf{Godspeed Scale for Human-Robot Interaction:} We measured students' social perception in SAMI by using the Godspeed scale developed and empirically validated by~\citeauthor{bartneck2009measurement}. This scale has been widely used to measure user's social perception of AI agent in prior literature (e.g.,~\cite{wang2021towards}). This scale is a semantic differential scale that asks participant to indicate their position on a scale between two bipolar words (e.g., Fake 1 2 3 4 5 Natural). Given that some of the dimension measurements are only applicable to robots (e.g., animacy and perceived safety), we adapted the scale and only took the three dimension measurements that are applicable to SAMI:~\textit{Anthropomorphism, Perceived Intelligence, and Likeability.}~\textit{Anthropomorphism} measures participants' level of attribution of human forms or human characteristics to the agent;~\textit{Perceived Intelligence} measures participants' perception of how smart or intelligent the agent is;~\textit{Likeability} measures participants' level of positive impression of the agent. A score for each dimension was calculated by taking the average of participants' reported score of statements with the corresponding dimension. 

